A Hamilton-Jacobi Reachability-Based Framework for Predicting and Analyzing Human Motion for Safe Planning

Real-world autonomous systems often employ probabilistic predictive models of human behavior during planning to reason about their future motion. Since accurately modeling human behavior a priori is challenging, such models are often parameterized, enabling the robot to adapt predictions based on observations by maintaining a distribution over the model parameters. Although this enables data and priors to improve the human model, observation models are difficult to specify and priors may be incorrect, leading to erroneous state predictions that can degrade the safety of the robot motion plan. In this work, we seek to design a predictor which is more robust to misspecified models and priors, but can still leverage human behavioral data online to reduce conservatism in a safe way. To do this, we cast human motion prediction as a Hamilton-Jacobi reachability problem in the joint state space of the human and the belief over the model parameters. We construct a new continuous-time dynamical system, where the inputs are the observations of human behavior, and the dynamics include how the belief over the model parameters change. The results of this reachability computation enable us to both analyze the effect of incorrect priors on future predictions in continuous state and time, as well as to make predictions of the human state in the future. We compare our approach to the worst-case forward reachable set and a stochastic predictor which uses Bayesian inference and produces full future state distributions. Our comparisons in simulation and in hardware demonstrate how our framework can enable robust planning while not being overly conservative, even when the human model is inaccurate.

==> (ICRA 2020) Reachability for Human Motion Predictors/macros.tex <==
\usepackage{times}
\usepackage{color, colortbl, xcolor}
\input{notation}
% \usepackage{cite}
% \usepackage[numbers]{natbib}
\usepackage{multicol}
\usepackage[bookmarks=true]{hyperref}
%\usepackage[draft]{hyperref}

\usepackage{amsfonts}
\usepackage{algorithmic}
\usepackage[ruled,vlined,titlenotnumbered]{algorithm2e} 
\usepackage{amsmath}
\usepackage{dsfont}
\usepackage{subfigure}
%\usepackage{caption}
\usepackage{multicol}
\usepackage[pdftex]{graphicx}   
\usepackage{graphicx}
%\usepackage{subcaption}
%\usepackage{cite}

\graphicspath{{./figs/}}    
% and their extensions so you won't have to specify these with    
% every instance of \includegraphics      
\DeclareGraphicsExtensions{.pdf,.png}  

\usepackage[textfont=md,font=footnotesize]{caption}

\usepackage[left=55pt, right=55pt, top=55pt, bottom=58pt]{geometry} 
% \usepackage{afterpage}

\IEEEoverridecommandlockouts
\overrideIEEEmargins

\usepackage{balance}

\usepackage[%
    style=numeric-comp,
    sorting=none,
    backend=biber,
    sortcites=true,
    doi=false,
    %url=false,
    firstinits=true,
    hyperref,
    isbn=false,
    eprint=false,
    %backref=true,
    maxcitenames=3, %How many people before *choosing* to contract with [et al.]
    minbibnames=3, %How many authors *at least*  before *inserting* the [et al.]
    maxbibnames=4, %How many authors *at most*  before *inserting* the [et al.]
    block=none]
    {biblatex}
    
    % Get rid of the "In:"
    \renewbibmacro{in:}{}
    % Don't display language
    \AtEveryBibitem{%
  	\clearlist{language}%
  	\clearfield{pages}%
	}
\bibliography{references}
\maxdeadcycles=500
% \addbibresource{references.bib}
\def\bibfont{\small}




%%%%%%%%%%

\usepackage{lipsum}

\newcommand\blfootnote[1]{%
  \begingroup
  \renewcommand\thefootnote{}\footnote{#1}%
  \addtocounter{footnote}{-1}%
  \endgroup
}
%%%%%%

\definecolor{planning_color}{RGB}{69, 174, 254}    
\definecolor{prediction_color}{RGB}{255, 116, 190}
    
\newcommand{\example}[1]%
{
\textbf{Running example:}
\textit{#1}
}

% Normal font for URLs
\renewcommand\UrlFont{\rmfamily}

% Command for notes
\usepackage{ifthen}
\newboolean{include-notes}
\setboolean{include-notes}{true}
\newcommand{\abnote}[1]{\textcolor{blue}{AB: #1}}
\newcommand{\SBnote}{\textcolor{red}}
\newcommand{\ernote}[1]{\textcolor{orange}{\textbf{ER: #1}}}
\newcommand{\adnote}[1]{\ifthenelse{\boolean{include-notes}}{\textcolor{purple}{{A (comment):#1}}}{}}   
\newcommand{\adedit}[1]{\ifthenelse{\boolean{include-notes}}{\textcolor{magenta}{{A (edit):#1}}}{}}   

==> (ICRA 2020) Reachability for Human Motion Predictors/notation.tex <==
% Commands for mathematical notations

% Human notation
\newcommand{\hdyn}{f_H}
\newcommand{\hstate}{x_H}
\newcommand{\hderiv}{\dot{x}_H}
\newcommand{\hctrl}{u_H}
\newcommand{\cset}{\mathcal{U}}
\newcommand{\hxdim}{{n_H}}
\newcommand{\hudim}{{m_H}}

% Parameter notation
\newcommand{\param}{\lambda}
\newcommand{\belief}{P}
\newcommand{\pt}{\belief^{\tvar}}
\newcommand{\priorpt}{\belief^{\tvar}_{-}}
\newcommand{\postpt}{\belief^{\tvar}_{+}}
\newcommand{\pparam}{\belief(\param)}
\newcommand{\ptparam}{\pt(\param)}
\newcommand{\priorptparam}{\priorpt(\param)}
\newcommand{\postptparam}{\postpt(\param)}

% Joint human and parameter notation
\newcommand{\jointstate}{z}
\newcommand{\jointdyn}{f}
\newcommand{\betaintrdyn}{k}

% Robot notation
\newcommand{\rdyn}{f_R}
\newcommand{\rstate}{x_R}
\newcommand{\rderiv}{\dot{x}_R}
\newcommand{\rctrl}{u_R}
\newcommand{\rxdim}{n_R}
\newcommand{\rudim}{{m_R}}
\newcommand{\rgoal}{{g_R}}

% Environment notation
\newcommand{\map}{\mathcal{M}}

% Prediction notation
\newcommand{\predhor}{H}

% For control related stuff
\newcommand{\tvar}{t}
% \newcommand{\thor}{0} % Time horizon. could be t_f
\newcommand{\R}{\mathbb{R}}
% \newcommand{\ctrl}{u}
% \newcommand{\dstb}{d}
% \newcommand{\cfunc}{u(\cdot)}
% \newcommand{\dfunc}{d(\cdot)}
% \newcommand{\cset}{\mathcal{U}}
% \newcommand{\cfset}{\mathbb{U}}
% \newcommand{\dset}{\mathcal{D}}
% \newcommand{\dfset}{\mathbb{D}}
\newcommand{\state}{\jointstate}
% \newcommand{\traj}{\xi} 
% \newcommand{\dyn}{f} 
\newcommand{\targetfunc}{l}
\newcommand{\targetset}{\mathcal{L}}
% \newcommand{\costfunctional}{J}
% \newcommand{\costfunctionalBRS}{C}
% \newcommand{\costfunctionalBRT}{J}
\newcommand{\vfunc}{V}
% \newcommand{\brs}{\mathcal{V}} % backwards reachable set
\newcommand{\frs}{\mathcal{V}} % forward reachable set
\newcommand{\frspos}{\mathcal{K}} % FRS in the position space
\newcommand{\approxfrspos}{\tilde{\mathcal{K}}} % Approx. FRS in the position space
\newcommand{\proj}{\Pi}
% \newcommand{\warmfunc}{k}
% \newcommand{\stateinit}{\tilde{\state}}
% \newcommand{\tinit}{\tilde{\tvar}}
\newcommand{\ham}{H}
% \newcommand{\stateseq}{\bold{\state}}
% \newcommand{\ctrlseq}{\bold{\ctrl}}
% \newcommand{\totalcost}{\cost(\stateseq, \ctrlseq)}
% \newcommand{\pos}{p} % position
% \newcommand{\npos}{h} % non-position states
\newcommand{\tdummy}{\tau}
% \newcommand{\tdummyy}{s}
% \newcommand{\trajstandard}{\traj_{\state, \tdummy}^{\ctrl,\dstb}}

% Analysis stuff
\newcommand{\tmin}{T_{\text{min}}}
\newcommand{\tmax}{T_{\text{max}}}

% For navigation stuff
\newcommand{\env}{\mathcal{E}}
\newcommand{\planner}{\Pi}
\newcommand{\sense}{\mathcal{S}}
\newcommand{\initSafe}{\mathcal{X}_{\text{init}}}
\newcommand{\brsSafe}{\mathcal{W}}
\newcommand{\horizon}{T}
\newcommand{\planninghorizon}{H}
\newcommand{\finaltime}{\bar{T}}
\newcommand{\plannerSafe}{\planner^{*}}
\newcommand{\freeRegion}{\mathcal{F}}
\newcommand{\queue}{\mathcal{Q}}
\newcommand{\neighbor}{\mathcal{N}}
\newcommand{\timestep}{\Delta{T}}

% For general math stuff
\newcommand{\reals}{\mathbb{R}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
\newcommand{\argmin}{\operatornamewithlimits{argmin}}

% FRS notation
\newcommand{\frsname}{\text{BA-FRS}}

% For proof utilities
\newtheorem{remark}{Remark}
\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}

==> (ICRA 2020) Reachability for Human Motion Predictors/sections/analysis.tex <==
%\section{Utility of the Reachability-based Motion Prediction Framework}
\section{A New HJ Reachability-based Predictor} \label{sec:new_predictor}
Our reachability-based framework enables us generate a new predictor by computing an approximation of \frsname{}.
% using the allowable human controls set for a future joint state $\jointstate$ to be those with high enough probability given $\jointstate$. 
In this section, we analyze the similarities and differences between this predictor and the one obtained by solving the full stochastic reachability problem.

\noindent\textbf{Prediction as an approximation of $\frspos$.}
Since the stochastic reachability problem needs to explicitly maintain the state probabilities, it might be challenging to compute $\frspos$ compared to $\approxfrspos$.
% Since the human motion often needs to be predicted at run time, $\approxfrspos$ thus allows for a more scalable prediction. 
However, this advantage in computation complexity is achieved at the expense of losing the information about the human state distribution, which can be an important component for several robotic applications.
However, when the full state distribution is not required, as is the case in this paper, $\approxfrspos$ provides a very good approximation of $\frspos$. 
In fact, it can be shown that $\frspos^{\tvar}_0(\tdummy) = \approxfrspos^{\tvar}_0(\tdummy)$.
% \adnote{explain here how it relates, use running example}
\example{
% When $\epsilon$ and $\delta$ are non-zero, the theoretical relationship between the two sets depends on the human policy and the initial belief; however, we now empirically demonstrate that $\approxfrspos^{\tvar}(\tdummy)$ still provides a good approximation of $\frspos^{\tvar}(\tdummy)$.
For simplicity, consider the case when the intrinsic behavior of the human does not change over time, i.e., $\betaintrdyn(\ptparam) = 0$. 
% We also let $\gamma = 1$.
Since in this case $\param$ takes only two possible values, the joint state space is three dimensional. 
In particular, $\jointstate = [h_x, h_y, p_1]$, where $p_1 := \belief(\param = g_1)$.
$\belief(\param = g_2)$ is given by $\left(1-\belief(\param = g_1)\right)$ so we do not need to explicitly maintain it as a state.
$P(\hctrl \mid \jointstate) = p_1 \mathcal{N}(\mu_1, \sigma_1^2) + (1 - p_1)\mathcal{N}(\mu_2, \sigma_2^2)$
%$P(\hctrl \mid \jointstate)$ is given by
%
%\begin{equation*}
%    P(\hctrl \mid \jointstate) = \frac{p_1}{\sqrt{2\pi\sigma^2_1}} e^{-\frac{(\hctrl - \mu_1)^2}{2\sigma^2_1}} + \frac{(1-p_1)}{\sqrt{2\pi\sigma^2_2}} e^{-\frac{(\hctrl - \mu_2)^2}{2\sigma^2_2}},
%\end{equation*}
%
which can be used to compute the set of allowable controls $\cset$ for different $\delta$s as per \eqref{eqn:jointdyn_HJ_controlpolicy}. 
% Recall that $\mu_1$ and $\mu_2$ are dependent on the human state, and hence the set of allowable controls is state dependent. 
% However, our reachability framework can easily handle this scenario.
We use the Level Set Toolbox \cite{mitchell2004toolbox} to compute the \frsname{}, starting from $\hstate = (0, 0)$.
The corresponding likely human states, $\approxfrspos^{\tvar}_{\delta}(\horizon)$, for different initial priors and $\delta$s are shown in Fig. \ref{fig:frs_illustration} in magenta.
For comparison purposes, we compute $\frspos^{\tvar}_{\epsilon}(\horizon)$ (teal), as well as the ``naive'' FRS obtained using all possible human actions (gray).
$\epsilon$ for $\frspos$ is picked to capture 95\% area of the set. \\
As evident from Fig. \ref{fig:frs_illustration}, $\approxfrspos^{\tvar}$ is an over-approximation of $\frspos^{\tvar}$, but at the same time it is not overly conservative unlike the naive FRS. 
This is primarily because even though the proposed framework doesn't maintain the full state distribution, it still discards the unlikely controls during the \frsname{} computation.
It is also interesting to note that \frsname{} is not too sensitive to the initial prior for low $\delta$s. 
This property of \frsname{} allows the predictions to be robust to incorrect priors as we explain later in this section. 
\\
We also show the full 3D \frsname{}, as well as the projected $\approxfrspos^{\tvar}$ sets over time for an initial prior, $p_1 = 0.8$, in Fig. \ref{fig:full_3D_sets}.
When $\delta$ is high, both the belief as well as the human states are biased towards the goal $g_1$ over time. 
When $\delta$ is high, only the actions that steer the human towards $g_1$ will be initially contained in the control set for the \frsname{} computation.
Moreover, propagating the current belief under these actions further reinforces the belief that the human is moving towards $g_1$.
As a result, the beliefs in the \frsname{} shift towards a higher $p_1$ over time.
On the other hand, when $\delta=0.1$, the human actions under $g_2$ are also contained in the control set, which leads to the belief and the human state shift in both directions (towards $g_1$ and $g_2$). 
% However, there is still more propagation towards $g_1$, as expected given the initial prior.
}

%
\begin{figure} [t!]
    \centering
    \includegraphics[width=0.9\columnwidth]{figs/bayes_bafrs_comparison_cropped.pdf}
    \caption{As $\delta$ increases, we obtain a tighter approximation of $\frspos^{\tvar}$; this is because a sequence of ``medium'' likely actions over time result in states that are overall unlikely under a Bayesian prediction. Discarding such actions under our framework leads to a better approximation of $\frspos^{\tvar}$. However, choosing $\delta$ too aggressively might lead to an overly optimistic set.}
    \label{fig:frs_illustration}
    \vspace{-2em}
\end{figure}
%


\noindent\textbf{Prediction as robust to incorrect priors and misspecified models.} 
% \adnote{stuff about misspecification}
% In this section, we illustrate some of the additional advantages of the proposed reachability-based prediction scheme.
% \subsection{Robustness to Incorrect Priors and Misspecified Models}
The set $\frspos^{\tvar}_{\epsilon}(\horizon)$ depends heavily on the prior $\ptparam$.
% Moreover, the corresponding $\epsilon$ that one needs to pick also depends heavily on this prior to make sure that $\frspos^{\tvar}(\cdot)$ is not too conservative or optimistic. 
When the initial prior for the human motion prediction is not accurate enough, using $\frspos^{\tvar}_{\epsilon}(\horizon)$ for planning might lead to unsafe behavior as it can be too optimistic.
This issue is particularly exacerbated when the true (unknown) parameter of the human, $\param^{*}$, is not within the support of $\param$ considered in the model, i.e., when the model is misspecified.
For example, when the exact goal of the human may not be any of the goals specified in the model.
In such scenarios, a full Bayesian inference may fail to assign sufficient probabilities to the likely states of the human, which can lead to unsafe situations.
On the other hand, using the \textit{full FRS}, i.e., the set of all states the human can reach under \textit{any} possible control, will ensure safety but can impede robot plan efficiency. 

In such situations, the proposed framework presents a good middle-ground alternative to the two approaches -- it does not rely heavily on the exact probability of an action while computing FRS since it leverages action probabilities only to distinguish between likely and unlikely actions.
Yet, it still uses a threshold to discard highly unlikely actions under the current belief, ensuring the obtained FRS is not too conservative.
This allows our framework to perform well in situations where the initial prior is not fully accurate but accurate enough to distinguish likely actions from unlikely actions.
In particular, suppose the prior at time $\tvar$ is such that $P(\hctrl \mid \hstate^\tvar; \param^{*}) \ge \delta \implies P(\hctrl \mid \jointstate^\tvar) \ge \delta ~\forall \hctrl$, 
% %
% \begin{equation} \label{eqn:robustness_condition}
% P(\hctrl \mid \hstate^\tvar; \param^{*}) \ge \delta \implies P(\hctrl \mid \jointstate^\tvar) \ge \delta ~\forall \hctrl,
% \end{equation}
% %
where $\param^{*}$ is the true (unknown) human parameter, and $\jointstate^\tvar = (\hstate^\tvar, \ptparam)$.
Intuitively, the above condition states that the prior at time $\tvar$ is accurate enough to distinguish the set of likely actions from the unlikely actions for the \textit{true} human behavior; however, we do not have the knowledge of the true probability distribution of the actions. 
In such a case, it can be shown that any human state that is reachable under a control sequence consisting of at least $\delta$-likely controls will be contained within $\approxfrspos^{\tvar}_{\delta}$. 

\example{Consider the scenario where the actual human goal is $g_3$, midway between $g_1$ and $g_2$ (see Fig. \ref{fig:misspecified_goal}). 
Thus, the current model does not capture the true goal of the human.
Even though the human walks straight towards $g_3$, a full Bayesian framework fails to assign sufficient probabilities to the likely human states because of its over reliance on the model.
Ultimately, this leads to a collision between the human and the robot.
In contrast, since our framework uses the model to only distinguish likely actions from unlikely actions, it recognizes that moving straight ahead is a likely human action.
This is also evident from Fig. \ref{fig:frs_illustration}, where the states straight ahead of the human are contained within the \frsname{} even for a relatively high $\delta$ of 0.2.
As a result, using the deterministic \frsname{} for planning leads to a safe navigation around the human. \\
These results are confirmed in our hardware experiments performed on a TurtleBot 2 testbed. As shown in Fig.~\ref{fig:front_fig}, we demonstrate these scenarios for navigating around a human participant. We measured human positions at ~200Hz using a VICON motion capture system and used on-board TurtleBot odometry sensors for the robot state measurement. As discussed, our framework allows us to be robust to misspecified goals while not being overly conservative. 
}
%
\begin{figure} [t!]
    \centering
    \includegraphics[width=0.8\columnwidth]{figs/planning_comparisons.pdf}
    \caption{Visualized is a snapshot of the human predictions $\frspos^{\tvar}_{\epsilon}(\horizon)$ starting from a prior of $(0.5, 0.5)$, and the corresponding trajectory of the robot when using the BA-FRS (left) or the Bayesian predictor (right).}
    \label{fig:misspecified_goal}
    \vspace{-2em}
\end{figure}
%

\section{Prediction Analysis} \label{sec:predictor_analysis}
% \adnote{modified into section, tweaked title}
% \adnote{i suggested an edit above where you would put the equation under that section (C), so remember to remove it from here and point back to that}
%One of the main objectives of Bayesian inference is to determine the true behavior of the human from a series of observations starting from a prior.
%Thus, one interesting question to ask is how much time (or equivalently the number of observations) will be required to determine the true human behavior under the current prior? Since our reachability based framework explicitly maintain all possible beliefs that are reachable under the current belief, it is well equipped to answer such questions.
% 
An interesting question that our framework can answer is how long does the predictor have to observe the human in order to determine the true human behavior for some prior.
% 
For simplicity, consider the scenario where $\param$ can take two possible values $b_1$ or $b_2$; however, the true human parameter is unknown.
We also have an initial prior over $\param$, given by $\belief^0(\param)$.
% Without loss of generality, suppose the true human parameter $\param^* = b_1$. 
Then we may pose the following questions: (1) What is the minimum and maximum possible time it will take to determine that $\param^* = b_1$ with sufficiently high probability (denoted as $\tmin^1$ and $\tmax^1$)? (2) What are the corresponding sequences of observations?
%two specific questions that could of interest:
%\begin{enumerate}
%    \item What is the minimum and maximum possible time it will take to determine that $\param^* = b_1$ with sufficiently high probability (denoted as $\tmin^1$ and $\tmax^1$)?
%    \item What are the corresponding sequences of observations? 
%\end{enumerate}
Thus, we want to know what is the most and the least informative set of observations that the human can provide under $\param^* = b_1$.
Similar questions can also be posed for $b_2$.
The overall minimum and the maximum time to determine the true human behavior are then given by $\tmin = \min\{\tmin^1, \tmin^2\}$ and $\tmax = \min\{\tmax^1, \tmax^2\}$.
Once $\tmin$ and $\tmax$ are available, the robot trajectory can be planned to safeguard against both possibilities ($\param^* = b_1$ and $\param^* = b_2$) for $\tvar \le \tmax$. 
After a duration of $\tmax$, we will be able to determine the true human behavior so it is sufficient to safeguard against the likely states of the human under the belief $\belief^{\tmax}(\param)$ there on.

As discussed in Sec. \ref{subsec:hj_framework}, an instantiation of the proposed reachability-based framework can be used to determine $\tmin$ and $\tmax$. 
In particular, given the initial human state $\hstate^0$ and the initial prior $\belief^0(\param)$, we can compute the \frsname{} with the control policy in \eqref{eqn:jointdyn_HJ_controlpolicy_gt},
% %
% \begin{equation}
%     \hctrl \in \cset,\quad \cset = \{\hctrl: P(\hctrl \mid \hstate; \beta_1) \ge \delta\},
% \end{equation}
% %
and the Hamiltonian $\ham(\tdummy, \state, \nabla \vfunc(\tdummy, \state)) = \max_{\hctrl \in \cset} \nabla \vfunc(\tdummy, \state) \cdot \jointdyn(\state, \hctrl).$
% 
% \begin{equation}
% \ham(\tdummy, \state, \nabla \vfunc(\tdummy, \state)) = \max_{\hctrl \in \cset} \nabla \vfunc(\tdummy, \state) \cdot \jointdyn(\state, \hctrl).
% \end{equation}
Then, $\tmin^1$ can be obtained as the minimum time such that $P^*_1(\param)$ is contained in $\frs(\cdot)$ for some human state $\hstate$.
Here, $P^*_1(\param)$ is a distribution that assigns a sufficiently high probability to $\param = b_1$.
Intuitively, this computation gives the minimum time it will take to reach the belief that $\param^* = b_1$ if the true human parameter is indeed $b_1$ and the human is giving us the most informative samples to discern its behavior.  
We can similarly compute $\tmin^2$ by computing a similar \frsname{} under the likely controls from $b_2$.

Similarly, $\tmax^1$ can be computed using a similar procedure, but instead of maximizing over the control in the Hamiltonian, we minimize over the control instead. 
This computation corresponds to finding the control sequence that is least informative at inferring $\param^* = b_1$ and can be obtained by: $
\hctrl^{*}(\tdummy,\jointstate) =  \arg \min_{\hctrl \in \cset} \nabla \vfunc(\tdummy, \jointstate) \cdot \jointdyn(\jointstate, \hctrl).
$
% 
% This computation corresponds to finding the set of joint states that the system will reach even when the human applies the control to minimize the growth of the \frsname{}.
% As a result, at $\tmax^1$, all possible trajectories that start from $\hstate^0$ and $\belief^0(\param)$ will reach the belief $P^*_1(\param)$ regardless of the control sequence applied by the human. 
% Consequently, within a duration of $\tmax^1$, we will be able to infer that the true human behavior is modeled by $b_1$, if that is indeed the case.
% The control sequence that is least informative at inferring $\param^* = b_1$ (and hence corresponds to the last state to reach the belief $P^*_1(\param)$) can be obtained as:
% %
% \begin{equation}
% \label{eq:opt_ctrl}
% \hctrl^{*}(\tdummy,\jointstate) =  \arg \min_{\hctrl \in \cset} \nabla \vfunc(\tdummy, \jointstate) \cdot \jointdyn(\jointstate, \hctrl).
% \end{equation}
%
Intuitively, $\hctrl^{*}$ is the control observation that least differentiate between $b_1$ and $b_2$. 
Similarly, $\hctrl^{*}$ corresponding to the computation of $\tmin$ is the control observation that differentiates most between $b_1$ and $b_2$. 
This is closely related to prior work on legibility \cite{dragan2013legibility} and deception \cite{dragan2014analysis}: given a fixed horizon, our framework computes a sequence of controls that is maximally informative or maximally ambiguous cumulatively across all the time steps, which in general is nontrivial to compute.
% Interestingly, the most informative sequence of actions for one hypothesis will not always coincide to the sequence of highest probability actions under that hypothesis -- this is the distinction between acting legibly and acting predictably -- which makes this informative sequence and the $\tmin$ nontrivial to compute.

\example{
Consider the planar pedestrian dynamics as before, but with the following human policy:
\begin{equation}
       \hctrl^{\tvar} \mid \hstate^{\tvar} \sim 
    \begin{cases}
        \mathcal{N}(0, \sigma^2),  & \text{if } \param = 0 \\
        \text{Uniform}(-\pi, \pi),  & \text{if } \param = 1,
    \end{cases} 
\end{equation}
where $\sigma = 0.1$. 
The human walks straight with a small variance when $\param = 0$ and move in a random direction when $\param = 1$, approximating an irrational human.
We compute the minimum and maximum time to realize $\lambda^* = 0$ starting from a high initial prior on irrational behavior, $(0.1, 0.9)$.
We assume that we can confidently conclude that $\lambda^* = 0$ when all human trajectories reach a belief of at least $0.9$ for $\lambda = 0$.
The obtained $\tmin$ and $\tmax$ are 3.2s and 11.2s respectively.
We also compute the control sequences that correspond to these times. 
The optimal control sequence for $\tmin$ is given by $\hctrl = 0$, since that is the most likely action under the rational behavior compared to irrational behavior.
On the other hand, for $\tmax$, the optimal control sequences consist of an angle of 15 degrees, which is the least likely action that is above the $\delta$-threshold (0.3 for this example) for $\lambda = 0$.
}


==> (ICRA 2020) Reachability for Human Motion Predictors/sections/background.tex <==
\section{Background}
%
\subsection{Hamilton-Jacobi Reachability}
\begin{itemize}
    \item (describe stuff about HJ reachability)
    \item Recall that our goal is to determine where the human will be in the future. More formally, we want to compute the set of all states that our human dynamical system can reach from the initial set of states $\mathcal{L}$ at time $T$. 
    \item This is a \textit{forward reachable set} computation and can be mathematically written as an intial-value PDE:
    \begin{align}
        \frac{\partial V}{\partial t} + \max_{\hctrl \in \mathcal{U}} \nabla_\hstate V(\hstate,t) \cdot \hdyn(\hstate,\hctrl) &= 0 \\
        V(\hstate, 0) &= l(\hstate(0)) 
    \end{align}
    where $\mathcal{L} = \{\hstate: l(\hstate(0)) \leq 0\}$ where $\hstate(0)$ is the initial human state.
\end{itemize}

\SBnote{
\begin{itemize}
    \item Computation of BRS.
\end{itemize}
}

%
\subsection{Inference of model confidence}
% \SBnote{
% \begin{itemize}
%     \item Setting -- a new measurement is received and the model parameters are updated.
%     \item Equation to update the parameters (Bayes rule).
% \end{itemize}
% }


\begin{itemize}
    \item Although $P(\hctrl_\tvar \mid \hstate_\tvar; \param)$ gives us some modeled structure on the human's behavior, choosing a fixed value of $\param$ may not capture the true behavior we observe. 
    \item Consider the scenario where $\param$ represents if a person is moving towards the door or towards a desk. If we fix the model to always assume that humans move towards doors, then when the human actually moves towards the desk, our predictor cannot assign sufficient probability to the human moving in that direction. Generally speaking, we will assume that do not know the true value of $\param$ beforehand. 
    \item Fortunately, we can estimate the likelihood of the person's $\param$ by observing their actions and performing Bayesian inference. Since we are uncertain about the true value of $\param$, we will place a distribution over $\param$ denoted $\ptparam$ where $\tvar$ indicates that this is the prior distribution over $\param$ at timestep $\tvar$. 
    \item Once we have a distribution over $\param$, we can measure the human's action, $\hat{\hctrl}$, online and treat this as evidence about what $\param$ value best explains the person's behavior. 
    \item Our model of the human's control policy $P(\hctrl_\tvar \mid \hstate_\tvar; \param)$ will let us understand how likely it is to observe $\hat{\hctrl}$ given the current state and a particular value of $\param$. This \textit{observation model} will be used to update $P_t(\beta)$ every time we receive a measurement via a Bayesian update:
    \begin{equation}
        P_{\tvar+1}(\param \mid \hctrl_\tvar, \hstate_\tvar) = \frac{P(\hctrl_\tvar \mid \hstate_\tvar; \param)P_{\tvar}(\param)}{\sum_{\bar{\param}} P(\hctrl_\tvar \mid \hstate_\tvar; \bar{\param})P_{\tvar}(\bar{\param})}
    \end{equation}
    \item The update of the distribution given the observed data can be thought of as the ``dynamics'' of the distribution over the $\beta$ parameter, where the data is the ``input'' to the dynamics. We will derive the exact form of the continuous-time dynamics later (note: how should we introduce this?)
\end{itemize}


==> (ICRA 2020) Reachability for Human Motion Predictors/sections/conclusion.tex <==
\section{Conclusion}% and Future Work}
When robots operate in complex environments around humans, they often employ probabilistic predictive models to reason about human behavior.
Even though powerful, such predictors can make poor predictions when the prior is incorrect or the observation model is misspecified. This in turn will likely cause unsafe behavior.
% While a full probabilistic prediction maybe tractable in some cases, it can be extremely difficult for agents whose intent and preferences are evolving over time.
In this work, we formulate human motion  prediction as a Hamilton-Jacobi reachability problem. 
We demonstrate that the proposed framework provides more robust predictions when the prior is incorrect or human behavior model is misspecified, can perform these predictions in continuous time and state using the tools developed for reachability analysis, and can be used for the predictor analysis. 
%Extending our methodology to multi-robot, multi-human settings as well as to other online learning-based settings are exciting future directions. %as well as to other application spaces such as manipulation.
% 
% and then present a Hamilton-Jacobi reachability-based framework that not only can compute an approximation of likely human states at a significant lower computational complexity, but can also perform predictor analysis.
% We demonstrate that the proposed framework also provides more robust predictions when the human behavior model is inaccurate, and demonstrate our approach in simulation and hardware.
% Extending our methodology to multi-robot, multi-human settings as well as to other online learning-based settings are exciting future directions. %as well as to other application spaces such as manipulation.


==> (ICRA 2020) Reachability for Human Motion Predictors/sections/intro.tex <==
\section{Introduction}
\begin{figure} [t!]
    \centering
    \includegraphics[width=0.8\columnwidth]{figs/front_fig.jpg}
    \caption{The robot models the human as walking towards one of the two goals shown in red. However, the human actually walks straight in between them. The predictions from our Hamilton-Jacobi reachability framework (center, in magenta) approximates the full probability distribution (right, in teal) while being more robust to model misspecification and less conservative compared to the naive full forward reachable set (left, in grey).}
    \label{fig:front_fig}
    \vspace{-1em}
\end{figure}

Planning around humans is critical for many real-world robotic applications. To effectively reason about human motion, practitioners often leverage predictive models of human motion during robot decision making. 
These models can be objective-driven where the human seeks to maximize an objective \cite{bai2015intention, baker2007goal, ng2000algorithms, ziebart2009planning, kitani2012activity} or pattern-based where the behavioral structure is learned from data and then used for planning around human arms \cite{amor2014interaction, ding2011human, koppula2013anticipating, lasota2015analyzing, hawkins2013probabilistic}, drivers \cite{hawkins2013probabilistic, Schmerling2017, driggs2018robust}, and pedestrians \cite{Ma_2017_CVPR, alahi2016social} (see \cite{rudenko2019human} for a detailed survey).
% 
%Such predictive models encode relevant structure in human decision-making---such as goal-seeking behavior or preferences for smooth motions---as model parameters.
Such predictive models often encode the relevant structure in human decision-making as model parameters. However, since modeling the true human behavior and how people make decisions \textit{a priori} is challenging, predictors maintain a belief distribution over these model parameters \cite{fisac2018general, lasota2017multiple}. 
This enables the predictor to use observations of human behavior during runtime to update the belief over the model parameters and probabilistically predict the human motion in accordance with the observations. 

% Unfortunately, probabilistic predictions over future human states is typically a computationally demanding task, made only more demanding if the predictive model encodes how the human's behavior\adnote{make it clear that you're referring to the internal state, and give an example to motivate why (someonemight change their goal or diriving style or what not)} may change over time; predictions now have to account for not only future observations\adnote{i find the term accounting for future observations confusing, as you have not established prediction has to account for future observations -- you've only said that predictions depend on past observations via belief, and that predictions may account for human internal state dynamics; i think here instead of account for future observations you mean reason about future actions given the current belief} but also all possible ways in which the true model parameters may evolve. 
%
Unfortunately, generating probabilistic predictions over future human states is typically computationally demanding, made only more demanding if the human behavior may change over time.
%For example, a person walking through a hallway may suddenly change course upon realizing they forgot an item of theirs.  
For example, a human driver might change how aggressive their driving style is over time, which needs to be accounted for during the predictions.
Consequently, the predictor must now reason about all possible ways in which the model parameters and the corresponding predicted future human actions may evolve, given the current belief. In practice, however, computing the full probabilistic predictions may not necessarily be required for planning. Instead, identifying a set of states that the human will occupy with sufficiently high probability can enable the robot to avoid collisions quickly and effectively using a variety of motion planning techniques that use deterministic obstacles \cite{yoder2016autonomous, koenig2005fast, bekris2007greedy, janson2018safe}. 

In this work, we formalize the human prediction problem as a stochastic reachability problem \cite{prandini2006stochastic, abate2008probabilistic, bujorianu2007new, hu2000towards} in the joint state space of the human and the belief over the predictive model parameters.
Using this formulation, the full state distribution can be computed via a stochastic forward reachable set \cite{vinod2018stochastic, abate2007computational}, which is the set of all states and beliefs that are reachable under the human policy with at least a given probability threshold.  
However, instead of computing the stochastic reachable set, we present a novel Hamilton-Jacobi (HJ) reachability-based framework for computing a deterministic approximation of the set of probable states. 
We do so by restricting the human policy to a deterministic set of allowable actions. 
This not only allows us to predict likely human states with a significantly lower computational complexity, but it also gives rise to a general framework wherein different definitions of allowable human actions can be instantiated to (a) generate predictions and (b) perform predictor analysis. 

In particular, for prediction, the allowable human actions are those that have high enough probability with respect to any given state and belief. 
Since we do not explicitly maintain the state probabilities during prediction, on one hand our framework may lead to conservative predictions. 
On the other, our predictions are not too sensitive to these probabilities and are robust to misspecified belief distributions and model parameters (see Figure \ref{fig:front_fig}). 

Our framework additionally enables predictor analysis. 
For example, a robot motion planner might need to know how long it will take the predictor to correct a wrong prior given a hypothesized ground truth value of the human model parameters, or to disambiguate between competing hypotheses. 
We can readily answer such questions by instantiating the allowable human actions (which we use for computing our reachable sets) to model specific ground truth parameters' values. 
For instance, when the model parameter represents potential human goal locations, we can compute how long it would take a predictor to realize that the human is going towards a specific goal in the scene. 
If we do this for two goals in the scene and take the maximum of those times, the robot now also knows that no matter which of the two goals the human is actually pursuing, the identity of the correct goal will become clear within that amount of time.
% 
% We can readily answer such questions by restricting allowable human actions to model the hypothesized ground truth, and compute how long  it takes the predictor to correct an incorrect prior. 
% 
% \adnote{this paragraph needs some work to both explain why restricting allowable actions to model a hypothesized ground truth relates to questions you raised, as well as to incorporate the disambigutation properly (the last sentence now talks aabout correcting a n incorrect prior only}\adnote{e.g. "how long it will take for the predictor to correct a wrong prior given a hypothesized ground truth value for human internal state, or to disambiguate between competing hypotheses. We can readily answer such questions by instantiating the allowable human actions (which we use for computing our reachable sets) to model specific ground truth internal state values. For instance, we can compute how long it would take a predictor to realize that the human is going towards a specific goal. If we do this for two goals in the scene and take the maximum of those times, the robot now also knows that regardless which of the two goals the human is pursuing, the identify of the correct goal will become obvious within that amount of time."}

\ernote{We should probably defer the following discussion of comparing our approach with POMDPs and belief state MDPs, to e.g. the journal version.} Our framework can also be thought of as a marriage between techniques from the belief space planning literature, and optimal control methods. For example, POMDPs are often recast as belief space MDPs, which in turn often admit more computationally efficient solution methods~\cite{kurniawati2008sarsop, roy2005finding, pineau2003point}. Similarly to how POMDPs can be recast as equivalent belief space MDPs, we also operate in belief space. But rather than doing both the planning and prediction in the belief space, we only do human motion prediction in the belief space, separate from planning, as is often done in the literature to reduce the computational complexity (e.g.~\cite{littman1995learning}). However, we use theoretically-rich continuous-time reachability analysis \cite{mitchell2005time, abate2008probabilistic} for prediction, which allows us to leverage a variety of tools \cite{mitchell2004toolbox, chen2013flow} developed to solve such problems grounded within the optimal control literature.  
%

To summarize, our key contributions are:
\begin{itemize}
    \item a Hamilton-Jacobi reachability-based framework for prediction generation and predictor analysis;
    \item demonstration of our approach in simulation and on a hardware testbed for safe navigation around humans.
\end{itemize}

% \abnote{Anca point: say "from the perspective of reachability people -- this is what our paper gives you. From the perspective of Bayesian prediction people -- this is what our paper gives you." We should do this both in intro and conclusion.}
% 
% \vspace{1cm}
% 
% \adnote{v0 [best of all words]}
% \begin{itemize}
%     \item planning requires human behavior prediction
%     \item human behavior is driven by human internal state: intentions, preferences; predictors can account for this by holding a belief over that internal state (cites)
%     \item this makes predicting probability distributions over future human states difficult especially if the human internal state is dynamic (e.g. if the person might change their goal): the robot has to not just account for possible future actions given an internal state, but also the possible ways in which the internal state might evolve
%     \item (all you need is a set:) often times though, what we use for safe planning is not the full probability distribution: what we care about is identifying a set of states that has high enough probability -- we want to avoid collisions with all of those, and do not necessarily need to know which states within that set are more or less probable
%     \item (insight: we can approximate the set via reachability) we observe that finding such a set of probable states is a simpler problem than finding a full distribution; our insight is that we can approximate this set by formalizing prediction as a reachability problem; this is no ordinary reachability problem though: it's one where we compute which states \emph{and beliefs} are reachable 
%   given certain assumptions on allowable human actions; 
%   \item importantly, even though we do reachability in belief space, this is still much simpler than the problem of finding the full distribution -- that'd be stochastic reachability, complexity XX, whereas ours has complexity XX
%   \item this gives us a framework: we can plug in different definitions for allowable human actions and get different results; 
%   \item 1) prediction:  by restricting allowable human actions given a state and belief to only those actions that have high enough probability with respect to that state and belief, we obtain a new predictor; we show that it approximates the set we'd obtain by first computing the full probability distribution and then selecting states with high enough probability; it sometimes differs, because it does not trust the probabilities from previous steps -- we end up with something less accurate if the human model giving us probabilities is correct, but more robust to misspecification of that model; overall, a good combination of the bayesian and the worst case! 
%   \item 2) for self-introspection: a planner might need to know how long it would take for the predictor to correct a wrong prior, or to be able to disambiguate between competing hypotheses; we can compute that using our framework by restricting the allowable human actions to have high enough probability given a specific value of human internal state,
%   \item contributions: framework, new predictor, analysis
% \end{itemize}

% v1 [prediction story, emphasizing stochastic->deterministic insight]
% \begin{itemize}
%     \item planning requires human behavior prediction
%     \item human behavior is driven by human internal state: intentions, preferences; predictors can account for this by holding a belief over that internal state (cites)
%     \item this makes predicting probability distributions over future human states difficult especially if the human internal state is dynamic (e.g. if the person might change their goal): the robot has to not just account for possible future actions given an internal state, but also the possible ways in which the internal state might evolve
%     \item (all you need is a set:) often times though, what we use for safe planning is not the full probability distribution: what we care about is identifying a set of states that has high enough probability -- we want to avoid collisions with all of those, and do not necessarily need to know which states within that set are more or less probable
%     \item (insight: we can approximate the set via reachability) we observe that finding such a set of probable states is a simpler problem than finding a full distribution; our insight is that we can approximate this set by formalizing prediction as a reachability problem; reachability enables us to compute which states and beliefs are reachable given certain assumptions on allowable human actions; we compute our predicted set by restricting allowable human actions given a state and belief to only those actions that have high enough probability with respect to that state and belief
%     \item we first cast it as a stochastic reachability, and simplify the human actions from a probability distribution to a set of allowable actions
%     \item we show that it approximates the set we'd obtain by first computing the full probability distribution and then selecting states with high enough probability; it sometimes differs, because it does not trust the probabilities from previous steps -- we end up with something less accurate if the human model giving us probabilities is correct, but more robust to misspecification of that model; overall, a good combination of the bayesian and the worst case! 
%     \item bonus: we keep track of future beliefs, so we can answer questions about what those beliefs might be under different hypotheses, e.g. how long it would take to correct a wrong prior; 
% \end{itemize}

% v2 [belief story]
% \begin{itemize}
%     \item planning requires human behavior prediction
%     \item human behavior is driven by human internal state: intentions, preferences; predictors can account for this by holding a belief over that internal state (cites)
%     \item our goal in this work is to provide a framework for reasoning about what the robot's future beliefs might be under different assumptions about human behavior; this is important in two ways: 
%     \item 1) for self-introspection: a planner might need to know how long it would take for the predictor to correct a wrong prior, or to be able to disambiguate between competing hypotheses; 
%     \item 2) for prediction itself: especially if the human internal state is dynamic (e.g. if the person might change their goal), predictions about future states depend, implicitly or explicitly, on future beliefs
%     \item insight: computing what beliefs we might reach is a reachability problem: compute reachable states and beliefs given allowable human actions; this gives us a framework: we can plug in different definitions for allowable human actions and get different results; 
%     \item by restricting human actions for a future state and belief to have high enough probability given that state and belief, we get a predictor that approximates the high enough probability future human states -- it sometimes differs, and when it does we end up with something less accurate if the human model giving us probabilities is correct, but more robust to misspecification of that model
%     \item by restricting human actions to have high enough probability given a specific value of human internal state, we can compute how long it would take for the predictor to identify that value as the correct one with high enough probability
%   \end{itemize} 

% v3 [belief story, motivation first]   
% \begin{itemize}
%     \item planning requires human behavior prediction
%     \item human behavior is driven by human internal state: intentions, preferences; predictors can account for this by holding a belief over that internal state (cites)
%     \item this makes prediction difficult, especially if the human internal state is dynamic (e.g. if the person might change their goal): predictions about future states depend, implicitly or explicitly, on future beliefs
%     \item future beliefs are also important for analyzing the predictor: computing properties like how long it would take, given the current belief which might be wrong, to realize with high enough probability that the true human internal state is x
%     \item insight: computing what beliefs we might reach is a reachability problem! [further, we don't necessarily care about with what probability we will reach those beliefs, so it can simplified to a deterministic reachability problem:] compute reachable states and beliefs given allowable human actions; this gives us a framework: we can plug in different definitions for allowable human actions and get different results; 
%     \item by restricting human actions for a future state and belief to have high enough probability given that state and belief, we get a predictor that approximates the high enough probability future human states -- it sometimes differs, and when it does we end up with something less accurate if the human model giving us probabilities is correct, but more robust to misspecification of that model
%     \item by restricting human actions to have high enough probability given a specific value of human internal state, we can compute how long it would take for the predictor to identify that value as the correct one with high enough probability
% \end{itemize}


% \adnote{high level / most important comments:}

% \begin{itemize}
%     \item \adnote{is the paper solving the prediction problem, or is the paper solving the "how to be safe but not overly safe" problem -- how to make predictions that are a bit more conservative but not too conservative, and how to figure out properties of your predictor that you can count on in planning;}
%     \begin{itemize}
%         \item \adnote{right now, the paper is written about solving the prediction problem, with the latter stuff (robust prediction to misspecification and analysis) just being bonus ("additional advantages") (also the problem statement is for the prediction problem, and the framework is solving the prediction problem -- note, the framework right now is not written as a framework, because it's a single thing -- i.e. the full on bayesian predictor, the fact that you can change it only becomes clear later in the last section on these "additional advantages");}
%         \item \adnote{ but really, we're computing the exact full bayesian predictor in the "framework", which begs the question -- is that useful on its own as the main contribution, rather than the main contribution being that we have a framework for these robustness/analysis "additional advantages"?}
%         \item  \adnote{if it is useful on its own, it'd be because it's an easier compute / possible for continuous spaces (which i don't get, because it's stochastic reachability) -- if it is useful for full on prediction, we should have the main "experiments" focus on that, i.e. show that you can compute the predictions when you couldn't before, or faster than you could before; }
%         \item \adnote{i worry we don't have that; instead, what we have is the latter stuff -- we have more robust prediction, and we have answers;}
%     \end{itemize}
       
% \item  \adnote{ to me right now, the contribution is towards the "how to be safe but not overly safe" instead; if so, we should be changing the problem statement to reflect this (by adding past the prediction problem which questions about the prediction we're trying to answer), as well as the intro and some of the language around where robust prediction and analysis get introduced        }
% \end{itemize} 

% \adnote{related: in intro and problem statement, the statement that we need to figure out what our future beliefs will be is taken for granted, but it's highly unclear why it's true; for the intro, i'd love to see a version where we make tracking future beliefs a goal in itself, motivated by a) dynamics of internal state, and b) being able to answer questions about your future belief, like when you will correct your prior if it's wrong, and when you will be able to differentiate between alternative hypotheses; then, once it's clear that we want to track future beliefs, we can say that our insight is to pose this as a reachability problem; we plug in different restrictions on what the human controls can be, and get different predictors and analysis answers out}


% Planning around humans is critical for many real-world robotic applications. 
% Generating robotic motion plans which safely avoid nearby humans is challenging since any such planning scheme needs to reason not only about the current state of the human, but also its possible \textit{future} states.
% Practitioners often leverage predictive models to reason about the human behavior which are subsequently used by the robot during decision making.
% Recently, there has been a surge of interest in predictive models that can adapt online based on observations of human behavior.
% Such predictors typically maintain a belief over the internal state of the human which enable richer predictions when certain parts of the human behavior is not known \textit{a priori} and must be inferred in real time.
% Even though powerful in their approach, such predictors also face some challenges: 
% since the predictor is adaptive, it is important to reason about how the belief itself might change due to the future observations\adnote{why????}.
% Moreover, the human internal state itself might change over time, which needs to be appropriately accounted for during the prediction.
% These challenges need to be overcome not only to predict the likely future states of the human, but also to reason about the convergence of the belief to the true human behavior in the scenarios where the predictor is either too conservative or not yet accurate enough to be trusted for the robotic decision making.

% In this work, we propose a Hamilton-Jacobi reachability-based framework that can overcome these challenges.
% Our framework simultaneously reasons about all possible changes in the predictor's belief over time due to the potential future observations or the intrinsic changes in the human behavior, and their effect on the resulting human states.\adnote{flip the last two sentences -- state the need first, then say our observation/insight is that this is a reachability problem}
% In particular, we compute a Forward Reachable Set (FRS) in the joint state space of the human and the belief, which is the set of all beliefs and human states that the predictor can deem likely under some permissible future observations\adnote{emphasize and connect to the next paragraph: by instantiating the framework with different versions of what are permissible future observations, you can generate different predictors and analyses; by restricting human future actions to only eliminate actions that are too inconsistent with the human's behavior so far, you get a predictor that is less conservative than FRS but more robust than a typical Bayesian predictor; by restricting human future actions to be consistent with a specific hypothesis you can compute how long it will take to correct a wrong prior, or how long it will take to disambiguate between two different hypotheses..} starting from the current belief and human state.
% One of the main advantages of our framework stems from the availability of a variety of modern numerical tools for computing reachable sets \cite{mitchell2004toolbox, chen2013flow}. \adnote{I think this is a little vague at this point -- maybe make the computational argument at the end, after you've made the argument that the framework is useful because it gives you different predictors and analyses}

% Once computed, this FRS gives us all possible likely future states of the human which can be used for safe planning around humans.\adnote{this downplays the fact that you can get a predictor that's in between optimistic bayes and overly-conservative full frs (which assumes worst case human--see comment above for a suggestion on how to fix this by talking about the ways to instantitate the framework)}
% Moreover, since we explicitly maintain all possible future beliefs, our framework is well equipped to answer some key questions about the predictor, such as what are the minimum and maximum times that it will take for the belief to converge to the true behavior of the human? 
% What are the corresponding future observations that the predictor must receive to arrive at such a decision?
% The answers to these questions can inform safe planning around humans.
% To summarize, our key contributions are:
%     \begin{itemize}
%         \item a Hamilton-Jacobi reachability-based framework to reason about all possible changes in a predictor and the human state in light of future observations;
%         \item demonstration of how the proposed framework facilitates human motion prediction and its analysis\adnote{its seems to refer to the motion, but actually it's about the prediction.. maybe it's about motion too..}, enabling safer planning around humans;  
%         \item demonstration of our approach in simulation and on a hardware testbed for safe autonomous navigation around humans in indoor environments.
%     \end{itemize}

% \begin{itemize}
%     \item Planning around humans is critical for many real-world robots, but it is challenging to do and has large safety implications for autonomous systems
%     \item Practitioners often leverage predictive models to reason about human behavior which are subsequently used by the robot during decision making
%     %\item However, innacuracies in predictive models can lead the robot to confidently make unsafe decisions
%     \item Recent interest in predictive models which can adapt online based on observations of human behavior has enabled richer predictions when certain parts of the human behavior is not known \textit{a priori} and must be inferred in real time
%     \item For safety purposes, it is important to reason about how the predictor itself may change over time, which is a computationally challenging problem. 
%     \item In this work, we propose a Hamilton-Jacobi reachability-based framework that simultaneously reasons about all possible changes in the predictor over time and its effect on the resulting human state predictions
%     \item This gives us all possible likely states of the human which can be used for safe planning
%     \item Furthermore, the same framework allows us to ensure safety in scenarios where the predictor is not yet accurate enough to be trusted during robotic decision-making
%     \item Finally, our framework can be applied to a variety of nonlinear continuous-time dynamics models \abnote{ask Claire about how to talk about the continualization of the $P(\param)$ dynamics}
%     %However, it is unclear how to ensure safety in scenarios where the predictor is not yet accurate enough to be trusted during robotic decision-making. Ensuring safety here becomes even more challenging due to the fact that the predictor itself may change over time.
%     \item In our reachability framework, we treat the unobserved human measurements as `input' to the system and how the predictor changes based on the data as part of the `dynamics'
%     \item To summarize, our contributions are:
%     \begin{itemize}
%         \item casting this problem in a reachability framework
%         \item demonstration of how the proposed framework facilitates predictor analysis that enables safer planning 
%         \item demonstration of our framework in simulation and hardware
%     \end{itemize}
% \end{itemize}



% \abnote{QUESTION: can we utilize or explain what $u*$ means as a result of optimizing the Hamiltonian? Would be super cool -- Anca mentions connection to legibility and that the minimum control is the most legible one}

% \abnote{Link to our project website: \href{https://abajcsy.github.io/hallucinate/}{https://abajcsy.github.io/hallucinate/}}
% \SBnote{Outline
% \begin{itemize}
%     \item Why safety is important for autonomous systems?
%     \item What is missing in the current works at a high level? -- either they don't take into account how the human behavior model might change (RSS line of work), or work under the assumption of adversarial intruder (full FRS), or consider the average case (POMDPs). Recursive planning feasibility for the robot is also not formally addressed.
%     \item What are we aiming to do in this paper (a cautiously optimistic framework -- we want to take into account our data to reduce the pessimism about the human behavior while still keeping in mind that the current belief might change in future).
%     \item How do we do it? -- we cast the belief propagation problem as a reachability problem in the state space of human and the model parameters.
%     \item Summarize the key contributions -- (a) a novel framework that bridges the gap between different approaches to safety analysis for human-robot interaction, (b) an algorithm for provably safe and recursively feasible autonomous navigation in the presence of humans, and (c) demonstrate of the framework in simulation and on a hardware testbed. 
% \end{itemize}
% }

==> (ICRA 2020) Reachability for Human Motion Predictors/sections/intro_new.tex <==

% \begin{itemize}
%     \item human prediction is important and we need good predictive models
%     \item parameterized models of human decision making are nice in prediction when we have uncertainty in how humans make decisions. To deal with uncertainty, its desirable to keep a distribution over these paraemters.
%     \item through this uncertainty, typically, these models are used in stochastic predictors 
%     \item these predictors are great because we can leverage data to update their distributions based on measurements to make the predictive model align better with reality
%     \item however, at prediction time these stochastic predictors rely on a good prior and on the exact probabilities in the observation model. Finally, they are computationally demanding when you add in complex models of human decision making (e.g. dynamic beta)
%     \item in contrast, optimal control perspective on prediction is the forward reachable set
%     \item the predictions are definitely robust because we dont have to rely on priors or observation models and we have good tools for computing these sets for continuous-time dynamical systems
%     \item however, because you can't leverage any data to update the model, you get very conservative predictions and can't leverage structure of distributions
%     \item in this work we seek a marriage between the two approaches to get a more robust predictor that can still leverage human behavioral data online to reduce conservativism in a safe way
%     \item we cast this problem as a HJ reach problem in joint human and parameter space. this leads us to a novel prediction framework. Also gives us predictor analysis.
% \end{itemize}

\section{Introduction}
\begin{figure} [t!]
    \centering
    \includegraphics[width=0.8\columnwidth]{figs/front_fig.jpg}
    \caption{The robot models the human as walking towards one of the two goals shown in red. However, the human actually walks straight in between them. The predictions from our Hamilton-Jacobi reachability framework (center, in magenta) approximates the full probability distribution (right, in teal) while being more robust to model misspecification and less conservative compared to the naive full forward reachable set (left, in grey).}
    \label{fig:front_fig}
    \vspace{-1em}
\end{figure}

Planning around humans is critical for many real-world robotic applications. To effectively reason about human motion, practitioners often couple dynamics models with human decision-making models to generate predictions that are used by the robot at planning time. Such predictors often model the human as an agent maximizing an objective \cite{bai2015intention, baker2007goal, ng2000algorithms, ziebart2009planning, kitani2012activity} or they learn human behavioral structure  from data \cite{Schmerling2017}. When coupled with robot motion planners, these human decision-making models have been successfully used in a variety of domains including manipulation \cite{amor2014interaction, ding2011human, koppula2013anticipating, lasota2015analyzing, hawkins2013probabilistic}, autonomous driving \cite{hawkins2013probabilistic, driggs2018robust}, and navigation \cite{Ma_2017_CVPR, alahi2016social} (see \cite{rudenko2019human} for a survey).

%Such predictive models often encode the relevant structure in human decision-making through model parameters. \ernote{I typically think of ``structure'' as being the mathematical function (e.g. the Boltzmann distribution), which in turn has parameters. Maybe we could re-phrase: .} 
Such predictive models are often parameterized to encode variations in decision-making between different people. However, since modeling human behavior and how people make decisions \textit{a priori} is challenging, predictors can maintain a belief distribution over these model parameters \cite{fisac2018general, lasota2017multiple}.
% This is well-suited for stochastic predictors which generate full-state distributions \cite{ziebart2009planning, bandyopadhyay2013intention, kochenderfer2010airspace} and naturally incorporate the model parameter uncertainty into future state uncertainty. 
This stochastic nature of the predictor naturally incorporates the model parameter uncertainty into future human state uncertainty~\cite{ziebart2009planning, bandyopadhyay2013intention, kochenderfer2010airspace}.
Importantly, once deployed, the robot can observe human behavior and update the distribution over the model parameters to better align its predictive model with the observations. 
    
% However, there are two key challenges with such stochastic predictors. 
% First, there exist limited computational tools to compute these predictions in continuous time and state, which may be important for safety-critical applications. 
% Secondly, and perhaps more crucially, to update the distribution and to generate predictions, stochastic predictors rely on priors and on  observation models. 
% Although these two components enable data and prior knowledge to improve the model, observation models are difficult to specify and the priors may be incorrect. When either is erroneous, then the state predictions will be erroneous as well, and the robot may confidently plan unsafe motions. %Furthermore, it takes non-zero time and observations to correct an incorrect prior -- with traditional stochastic predictors, the robot still relies on these predictions during this time despite the prediction inaccuracies. 

However, there are two key challenges with such stochastic predictors. 
First, to update the distribution and to generate predictions, stochastic predictors rely on priors and on observation models. 
Although these two components enable data and prior knowledge to improve the model, observation models are difficult to specify and the priors may be incorrect. When either is erroneous, then the state predictions will be erroneous as well, and the robot may confidently plan unsafe motions. 
Secondly, there exist limited computational tools to generate these stochastic predictions in continuous time and state, which may be important for safety-critical applications. 

To address the former challenge, researchers in the robust control community have looked into \textit{full forward reachable set} predictors, which compute the set of \textit{all possible} states that the human could reach from their current state \cite{mitchell2005time, driggs2018robust}. 
Unfortunately, because these predictors consider worst-case human behavior, the resulting predictions are overly conservative, do not typically leverage any data to update the human model, and they significantly impact the overall efficiency of the robot when used in practice. 

%To combat some of these issues, the robust optimal control perspective on prediction removes any reliance on data and explicit structure in the human decision-making model. That is, the human is modeled as taking \textit{any} action from a conservative set of controls. Combined with a dynamics model, the predictor generates a \textit{full forward reachable set}, or the set of \textit{all} states that the human could reach from their current state \cite{mitchell2005time, driggs2018robust}. These predictors do not rely on priors or observation models and the control theory community has developed strong theoretic and numerical tools for analyzing the continuous-time evolution of such models. Unfortunately, because these predictors consider worst-case human behavior, the resulting predictions are overly conservative, cannot leverage any data to update the human model, and they significantly impact the overall efficiency of the robot when used in practice. 

%In this work we cast the human motion prediction problem as a reachability problem, which allows us to make a novel connection between the robust optimal control community and the human prediction community.  


In this work we seek a marriage between stochastic prediction and robust control: a predictor which is more robust to misspecified models and priors, but can still leverage human behavioral data online to reduce conservatism in a safe way. To do this, we cast human motion prediction as a Hamilton-Jacobi (HJ) reachability problem \cite{mitchell2005time, abate2008probabilistic, lygeros2004reachability} in the joint state space of the human and the belief over the predictive model parameters.
Observations of the human are treated as continuous ``input'' into our new dynamical system and how the belief over the model parameters changes based on this data are part of the ``dynamics'' of the system. 
However, unlike stochastic predictors, we do not rely on the exact probability of an observation during the prediction. 
Rather, we divide the possible human observations under the current model in two disjoint sets of \textit{likely} and \textit{unlikely} observations, and compute the possible future human states by treating all likely enough observations as equally probable.
%Since we no longer rely on the exact observation probabilities, the resulting predictor ensures safe planning when priors are not correct but can still leverage human behavioral data online to reduce conservatism in a safe way, thus bridging stochastic predictors with the full forward reachable set. 
Since we no longer rely on the exact observation probabilities, the resulting predictor exhibits robustness to incorrect priors, while still leveraging human behavioral data to reduce conservatism online in a safe way. In doing so, our algorithm provides a bridge between stochastic predictors and predicting the full forward reachable set. %(Note that we are not ensuring anything about the robustness of the \emph{planning}, just the robustness of the prediction.)
Additionally, our reachability formulation allows us to leverage the computational tools developed for reachability analysis to predict future human states in continuous time and state \cite{mitchell2004toolbox, chen2013flow}.
% Using this novel reachability formulation, we demonstrate how to bridge stochastic predictors with the full forward reachable set. This allows us to explicitly reason about how incorrect priors can affect our predictions in the future. Additionally, our formulation allows us to leverage the computational tools developed for reachability analysis to predict future human states in continuous time and state \cite{mitchell2004toolbox, chen2013flow}. Our resulting predictor ensures safe planning when priors are not correct but can still leverage human behavioral data online to reduce conservativism in a safe way.

Interestingly, because HJ reachability is rooted in optimal control, our novel formulation also allows us to analyze human models which change online based on data. For example, we can now ask (and answer) questions like ``How long will it take the predictor to reach a desired level of confidence in its human model?'' As long as the robot does not have enough confidence in the human model, this information can be used to plan safe maneuvers. 
Once the confidence in the human model is high enough, the robot can plan more aggressive maneuvers to improve performance.
%in light of a wrong prior given a hypothesized ground truth value of the human model parameters, or to disambiguate between competing hypotheses. We can readily answer such questions by instantiating the allowable human ``input'' to model specific ground truth parameters' values.


%To do this, we formalize the human prediction problem as a stochastic reachability problem \cite{prandini2006stochastic, abate2008probabilistic, bujorianu2007new, hu2000towards} in the joint state space of the human and the belief over the predictive model parameters. %Using this formulation, the full state distribution can be computed via a stochastic forward reachable set \cite{vinod2018stochastic, abate2007computational}, which is the set of all states and beliefs that are reachable under the human policy with at least a given probability threshold.  
%However, instead of computing the stochastic reachable set, we present a novel Hamilton-Jacobi (HJ) reachability-based framework for computing a deterministic approximation of the set of probable states. 
%We do so by restricting the human policy to a deterministic set of allowable actions. We use theoretically-rich continuous-time reachability analysis \cite{mitchell2005time, abate2008probabilistic} for prediction, which allows us to leverage a variety of tools \cite{mitchell2004toolbox, chen2013flow} developed to solve such problems grounded within the optimal control literature.
%This not only allows us to predict likely human states with a significantly lower computational complexity, but it also
%This gives rise to a general framework wherein different definitions of allowable human actions can be instantiated to (a) generate predictions and (b) perform predictor analysis. 

%In particular, for prediction, the allowable human actions are those that have high enough probability with respect to any given state and belief. Since we do not explicitly maintain the state probabilities during prediction, on one hand our framework may lead to conservative predictions. On the other, our predictions are not too sensitive to these probabilities and are robust to misspecified belief distributions and model parameters (see Figure \ref{fig:front_fig}). 


%Furthermore, our framework additionally enables predictor analysis. For example, a robot motion planner might need to know how long it will take the predictor to correct a wrong prior given a hypothesized ground truth value of the human model parameters, or to disambiguate between competing hypotheses. We can readily answer such questions by instantiating the allowable human actions (which we use for computing our reachable sets) to model specific ground truth parameters' values. For instance, when the model parameter represents potential human goal locations, we can compute how long it would take a predictor to realize that the human is going towards a specific goal in the scene. 
%If we do this for two goals in the scene and take the maximum of those times, the robot now also knows that no matter which of the two goals the human is actually pursuing, the identity of the correct goal will become clear within that amount of time.

%\ernote{We should probably defer the following discussion of comparing our approach with POMDPs and belief state MDPs, to e.g. the journal version.} Our framework can also be thought of as a marriage between techniques from the belief space planning literature, and optimal control methods. For example, POMDPs are often recast as belief space MDPs, which in turn often admit more computationally efficient solution methods~\cite{kurniawati2008sarsop, roy2005finding, pineau2003point}. Similarly to how POMDPs can be recast as equivalent belief space MDPs, we also operate in belief space. But rather than doing both the planning and prediction in the belief space, we only do human motion prediction in the belief space, separate from planning, as is often done in the literature to reduce the computational complexity (e.g.~\cite{littman1995learning}). However, we use theoretically-rich continuous-time reachability analysis \cite{mitchell2005time, abate2008probabilistic} for prediction, which allows us to leverage a variety of tools \cite{mitchell2004toolbox, chen2013flow} developed to solve such problems grounded within the optimal control literature.
%

To summarize, our key contributions in this work are:
\begin{itemize}
    \item a Hamilton-Jacobi reachability-based framework for human motion prediction which provides robustness against misspecified observation models and priors;
    %to design a predictor which is more robust to incorrect priors  when priors are not correct but can still leverage human behavioral data online whenever safe;
    \item a demonstration of how our framework can be used to analyze human decision-making models that are updated online;
    %\ernote{Maybe let's swap the order of the first two-- introducing it as a HJ reachability framework for doing analysis, and then present the predictor that comes out as an additional benefit}
    \item a demonstration of our approach in simulation and on hardware for safe navigation around humans.
\end{itemize}


==> (ICRA 2020) Reachability for Human Motion Predictors/sections/plan_our_approach.tex <==
\section{Our Approach: Planning}
%
\subsection{Human motion prediction for planning}
\SBnote{
\begin{itemize}
    \item Projection of the FRS on the beta dimension.
    \item Computation of the BRS for the planning purposes and why that is important.
\end{itemize}
}

%
\subsection{Safe online planning under uncertain human prediction}
\SBnote{
\begin{itemize}
    \item Planning given the states to be avoided.
    \item Update in the human model.
    \item Replanning.
    \item Lemma: Recursive feasibility.
\end{itemize}
}

==> (ICRA 2020) Reachability for Human Motion Predictors/sections/pred_our_approach.tex <==
\section{Reachability-based Motion Prediction}
%In general, computing $\frspos^{\tvar}_{\epsilon}(\cdot)$ is a computationally challenging problem.
%Thereby, we propose a reachability-based framework to compute these sets.  
In this section, we first discuss how to cast the full probabilistic human motion prediction problem as a stochastic reachability problem.
Next, we discuss how we can obtain a deterministic approximation of this stochastic reachability problem, and solve it using our HJ reachability framework.
% and then discuss HJ reachability analysis, a framework to solve this reachability problem. \adnote{add something about the stochastic first, deterministic but over belief after}
% 
% \begin{itemize}
%     \item We formulate prediction over human state and $P(\param)$ as a reachability problem
%     \item We define a new joint state space and dynamics
%     \item This problem can be solved via some powerful numerical approaches
% \end{itemize}

\subsection{Casting prediction as a reachability problem}
\label{sec:stochastic_fromulation}
% \adnote{this is starting too abruptly, needs some setup}
% \adedit{We cast the problem of predicting a probability distribution over human states as some future time as one of maintaining a time-dependent distribution over reachable states and beliefs, given a stochastic human model as in (refer to eq 2).}
We cast the problem of predicting a probability distribution over the human states at some future time as one of maintaining a time-dependent distribution over reachable states and beliefs, given a stochastic human model as in \eqref{eq:control_policy}. Let the current time be $\tvar$ with the current (known) human state $\hstate^{\tvar}$ and a belief $\ptparam$. 
Different control actions $\hctrl^{\tvar}$ that the human might take next will induce a change in both the human's physical state and the robot's belief over $\param$. This in turn affects what human action distribution the robot will predict for the following timestep, and so on.
To simultaneously compute all possible future beliefs over $\param$ and corresponding likely human states, we consider the joint dynamics of $\ptparam$ and the human:
%
\begin{equation} \label{eq:joint_dynamics}
\dot{\jointstate}^{\tvar} = [\dot{x}_{H}^{\tvar}~~ \dot{\belief}^{\tvar}(\param)]=  \jointdyn({\jointstate}^{\tvar}, \hctrl^{\tvar}). 
                % = \begin{bmatrix}
                % \hdyn(\hstate^{\tvar}, \hctrl^{\tvar}) \\
                % \gamma \left(\postpt(\param | \hctrl^\tvar) - \ptparam\right) + \betaintrdyn(\ptparam)
                % \end{bmatrix}
\end{equation}
%
At any state $\jointstate$, the distribution over the (predicted) human actions is given by
%
\begin{equation} \label{eqn:jointdyn_controlpolicy}
    \hctrl \sim P(\hctrl \mid \jointstate) = \displaystyle\sum\nolimits_{\bar{\param}}P(\hctrl \mid \hstate; \bar{\param})\belief(\bar{\param}).
\end{equation}
%

To derive the dynamics of $\ptparam$ in \eqref{eq:joint_dynamics}, we note that the belief can change either due to the the new observations (via the Bayesian update in \eqref{eqn:bayesian_update}) or the change in human behavior (modeled via the parameter $\param$) over time. 
% there could be two sources of changes in the belief: (a) the new observations can potentially change this distribution via the Bayesian update (see \eqref{eqn:bayesian_update}), and (b) the human behavior (modeled via parameter $\param$) itself might change over time. 
This continuous evolution of $\ptparam$ can be described by the following equation:
%
% \begin{equation} \label{eqn:beta_dynamics}
%     \dot{\pt}(\param) = \gamma \left(\postpt(\param | \hctrl^\tvar) - \ptparam\right) + \betaintrdyn(\ptparam).
% \end{equation}
\begin{equation} \label{eqn:beta_dynamics}
    \dot{\belief}^{\tvar}(\param) = \gamma \Big(\postpt(\param \mid \hctrl^\tvar, \hstate^\tvar) - \ptparam\Big) + \betaintrdyn\Big(\ptparam\Big).
\end{equation}
%
Here, the function $\betaintrdyn$ represents the intrinsic changes in the human behavior, whereas the other component captures the Bayesian change in $\ptparam$ due to the observation $\hctrl^\tvar$. 
% \adnote{i'm not really familiar with this notation, not sure what $\gamma$ does}
Note that the time derivative in \eqref{eqn:beta_dynamics} is pointwise in the $\param$ space.

Typically, the Bayesian update is performed in discrete time when the new observations are received; however, in this work, we reason about continuous changes in $\ptparam$ and the corresponding continuous changes in the human state.
We omit a detailed derivation, but intuitively, to relate continuous-time Bayesian update to discrete-time version, $\gamma$ in \eqref{eqn:beta_dynamics} can be thought of as the observation frequency. 
Indeed, as $\gamma \uparrow \infty$, i.e., observations are received continuously, $\ptparam$ instantaneously changes to $\postpt(\param \mid \hctrl^\tvar, \hstate^\tvar)$. 
On the other hand, as $\gamma \downarrow 0$, i.e., no observation are received, the Bayesian update does not play a role in the dynamics of $\ptparam$.
% For a detailed derivation of continuous dynamics, we refer the interested readers to \cite{XYZ}.
% Sec. \ref{subsec:beta_dynamics}. 

% \adnote{I'd move this paragraph up before getting into the belief dynamics, and I'd first talk about state z and then about the dynamics of the state f; note: one issue with the current phrasing is that it sounds like a thing that the human actually would phystically do, rather than the algorithm reasoning about possible future human actions and the resulting changes in belief that we have at time t for time t+1; here's an edit:}
% \adedit{We start at the current time t with the current human state xt and a current belief pt(beta). Different control actions  $\hctrl^{\tvar}$ that the human might take next induce a change in both state and belief, which in turn affect what action distribution we predict for the following timestep, and so on. }
% Suppose human applies a control action $\hctrl^{\tvar}$ at time $\tvar$. 
% This will change both the belief distribution over $\param$, ${\belief}^{\tvar}(\param)$, as well as the human state $\hstate^{\tvar}$.
% This change in belief distribution in turn affects the control actions that are likely at the next time instant, which in turn affects the next likely states of the human, and so on.
% To simultaneously compute all possible future beliefs over $\param$ and corresponding likely human states, we consider the joint dynamics of $\ptparam$ and the human:
% %
% \begin{equation} \label{eq:joint_dynamics}
% \dot{\jointstate}^{\tvar} = \begin{bmatrix}
%                 \dot{x}_{H}^{\tvar} \\
%                 \dot{\belief}^{\tvar}(\param)
%                 \end{bmatrix} =  \jointdyn({\jointstate}^{\tvar}, \hctrl^{\tvar}). 
%                 % = \begin{bmatrix}
%                 % \hdyn(\hstate^{\tvar}, \hctrl^{\tvar}) \\
%                 % \gamma \left(\postpt(\param | \hctrl^\tvar) - \ptparam\right) + \betaintrdyn(\ptparam)
%                 % \end{bmatrix}
% \end{equation}
% %
% At any state $\jointstate$, the set of allowable\adnote{not yet set of allowable, it's a distribution} human controls are given by
% %
% \begin{equation} \label{eqn:jointdyn_controlpolicy}
%     \hctrl \sim P(\hctrl \mid \jointstate) = \sum_{\param^{'}}P(\hctrl \mid \hstate; \param^{'})\belief(\param^{'})
% \end{equation}
%
%\adnote{i'd present this as a framework, where this is the thing different people should instantiate differently depending on what they need; for full prediction it's the above; for robustness its something else, for analysis it's something else.. }\adnote{nevermind, the framework part should go into C}

Given the joint state at time $\tvar$, ${\jointstate}^{\tvar}$, and the control policy in \eqref{eqn:jointdyn_controlpolicy}, we are interested in computing the following set:
%
\begin{equation}
    \frs(\tdummy) = \{\jointstate^{\tdummy} \mid P(\jointstate^{\tdummy} \mid \jointstate^{\tvar}) > 0\}, \tdummy \in [\tvar, \tvar + \horizon].
\end{equation}
%
Intuitively, $\frs(\tdummy)$ represents all possible states of the joint system, i.e., all possible human states and beliefs over $\param$, that are reachable under the dynamics in \eqref{eq:joint_dynamics} for some sequence of human actions.
We refer to this set as \textit{Belief Augmented Forward Reachable Set (\frsname)} from here on.
Given a \frsname, we can obtain $\frspos^{\tvar}(\tdummy)$ by projecting $\frs(\tdummy)$ on the human state space. In particular,
%
\begin{equation}
    \frspos^{\tvar}(\tdummy) = \bigcup_{\jointstate^{\tdummy} \in \frs(\tdummy)} \proj(\jointstate^{\tdummy}),~~\tdummy \in [\tvar, \tvar + \horizon],
\end{equation}
%
where $\proj(\jointstate)$ denotes the human state component of $\jointstate$.
Consequently, the probability of any human state can be obtained as $P(\hstate^{\tdummy}) = \sum_{\jointstate^{\tdummy} \in \frs(\tdummy)} P(\jointstate^{\tdummy} \mid \jointstate^{\tvar}), \text{ if}~ \hstate^{\tdummy} = \proj(\jointstate^{\tdummy})$ (and $0$ otherwise) 
%
% \begin{equation}
%     P(\hstate^{\tdummy}) = 
%         \begin{cases}
%             \sum_{\jointstate^{\tdummy} \in \frs(\tdummy)} P(\jointstate^{\tdummy} \mid \jointstate^{\tvar}),& \text{if}~ \hstate^{\tdummy} = \proj(\jointstate^{\tdummy})\\
%             0,& \text{otherwise}, 
%         \end{cases}
% \end{equation}
%
which can be used to obtain $\frspos^{\tvar}_{\epsilon}(\tdummy)$ for any $\epsilon \ge 0$.
%
% \begin{remark}
% Even though theoretically powerful, the reachability formulation presented in this section, can be computationally prohibitive for real-world systems. 
% However, when $\param$ takes some small number of discrete values, modern computational tools can be used to solve this reachability problem, as we illustrate later in this paper.\adnote{this remark belongs in the deterministic framework!}
% \end{remark}

Since the control policy in \eqref{eqn:jointdyn_controlpolicy} is stochastic, the computation of $\frs(\tdummy)$ is a stochastic reachability problem.
However, when the prior $\ptparam$ is not correct, safeguarding against $\frs(\tdummy)$ is not sufficient.
Moreover, even when the prior is correct, computing stochastic reachable sets can be computationally demanding \cite{abate2007computational}.
To overcome these challenges, we recast the computation of $\frs(\tdummy)$ as a \textit{deterministic} reachability problem.
We next discuss HJ-reachability analysis for computing the \frsname{}
thanks to modern computational tools \cite{mitchell2004toolbox, chen2013flow}, and discuss how we can cast $\frs(\tdummy)$ as a deterministic reachability problem.
% 
% 
% Since the control policy in \eqref{eqn:jointdyn_controlpolicy} is stochastic, the computation of $\frs(\tdummy)$ is a stochastic reachability problem which can be computationally demanding \cite{abate2007computational}. 
% % whose computational complexity typically scales exponentially in the dimension of $\hctrl$ \cite{XYZ}. 
% To overcome this challenge, we instead compute an approximation of $\frs(\tdummy)$, which can be obtained as the solution of a \textit{deterministic} reachability problem, significantly alleviating the computational complexity of $\frs(\tdummy)$ at the expense of obtaining more conservative predictions.
% We next discuss HJ-reachability analysis for computing the \frsname{}
% thanks to modern computational tools \cite{mitchell2004toolbox, chen2013flow}, and discuss how we can cast $\frs(\tdummy)$ as a deterministic reachability problem.
% 
% \begin{itemize}
%     \item Our predictive model is updated online based on measured data -- Given the possible future measurements of the person's actions, how will our predictions change? 
%     \item We will formulate this question as a reachability problem, wherein the future measurements are treated as ``input'' to the system and how the predictor changes based on the data are part of the ``dynamics'' of the system. The resulting forward reachable set will precisely capture the joint evolution of the human predictions \textit{and the predictor itself} over the prediction horizon.
%     \item Taking the reachability perspective will allow us to not only predict the future physical states of the human but also the evolution of the predictor given all possible human actions that we could observe in the future. (Note here: It also allows us to ask interesting analysis questions like min/max time it will take for our predictor to figure out the true human $\param$, etc.)
%     \item For our reachability computation, we want to know what physical states our predictor will mark as occupied by the human \textit{under all possible future distributions over} $\param$. To capture the evolution of both the human state and the predictor, we can combine the physical states of the human with the distribution over the parameter we are trying to estimate from measurements:
%         \begin{equation}
%             \jointstate_\tvar = \begin{bmatrix}
%                                 \hstate_\tvar \\
%                                 P_\tvar(\param)
%                                 \end{bmatrix}
%         \end{equation}
%     \item We can also combine the dynamics of the human with the dynamics of the distribution:
%         \begin{equation}
%             \dot{\jointstate}_\tvar = \jointdyn(\jointstate_\tvar, \hctrl_\tvar) = \begin{bmatrix}
%                     \dot{\hstate}_\tvar \\
%                     \dot{P}_\tvar(\param)
%                     \end{bmatrix} 
%                     \label{eq:joint_dynamics}
%         \end{equation}
%     \item Our new \textit{forward reachable set} computation and is now
%         \begin{align}
%             \frac{\partial V}{\partial \tvar} + \max_{\hctrl \in \mathcal{U}} \nabla_\jointstate V(\jointstate,\tvar) \cdot \jointdyn(\jointstate, \hctrl) &= 0 \\
%             V(\jointstate, 0) &= l(\jointstate(0)) 
%         \end{align}
%         where $z(0) = \begin{bmatrix}
%             x_0 \\
%             P_0(\beta = 0)
%         \end{bmatrix}$ and $\mathcal{L} = \{z: l(z(0)) \leq 0\}$ where $x_0$ is the initial human state measurement and $P_0(\beta = 0)$ is the predictor's initial prior over the human's $\beta$.
%     \item \abnote{NEED TO DESCRIBE SOMEWHERE HOW WE UPDATE THE DISTRIBUTION!}
% \end{itemize}

\begin{figure} [t!]
    \centering
    \includegraphics[width=\columnwidth]{figs/bafas_two_deltas.pdf}
    \caption{Visualization based on the the running example of the full BA-FRS and their projections into the human state space in the $h_x$-$h_y$ plane.}
    \label{fig:full_3D_sets}
    \vspace{-2em}
\end{figure}

\subsection{Background: Hamilton-Jacobi Reachability} \label{subsec:hj_reachability}
% \begin{itemize}
%     \item \abnote{put here the standard setup for reachability}
%     \item Recall that our goal is to determine where the human will be in the future. More formally, we want to compute the set of all states that our human dynamical system can reach from the initial set of states $\mathcal{L}$ at time $T$. 
%     \item This is a \textit{forward reachable set} computation and can be mathematically written as an intial-value PDE:
%     \begin{align}
%         \frac{\partial V}{\partial t} + \max_{\hctrl \in \mathcal{U}} \nabla_\hstate V(\hstate,t) \cdot \hdyn(\hstate,\hctrl) &= 0 \\
%         V(\hstate, 0) &= l(\hstate(0)) 
%     \end{align}
%     where $\mathcal{L} = \{\hstate: l(\hstate(0)) \leq 0\}$ where $\hstate(0)$ is the initial human state.
% \end{itemize}
% We use HJ reachability analysis to compute a forward reachable set (FRS) $\frs(\tdummy)$ given a set of starting states $\targetset$ \cite{lygeros2004reachability, mitchell2005time, bansal2017hamilton}.
% This analysis has been successfully applied in a variety of domains, such as aircraft auto-landing and safe large-scale multi-vehicle path planning \cite{bansal2017safe, bansal2017hamilton}.
HJ-reachability analysis \cite{lygeros2004reachability, mitchell2005time, bansal2017hamilton} can be used for computing a general Forward Reachable Set (FRS) $\frs(\tdummy)$ given a set of starting states $\targetset$.
Intuitively, $\frs(\tdummy)$ is the set of all possible states that the system can reach at time $\tdummy$ starting from the states in $\targetset$ under some permissible control sequence.
The computation of the FRS can be formulated as a dynamic programming problem which ultimately requires solving for the value function $\vfunc(\tdummy,\state)$ in the following initial value Hamilton Jacobi-Bellman PDE (HJB-PDE):
% %
% \begin{equation}
% \label{eq:HJB_FRS}
% \begin{aligned}
% &D_{\tdummy} \vfunc(\tdummy, \state) + \ham(\tdummy, \state, \nabla \vfunc(\tdummy, \state)) = 0, \\
% &\vfunc(0, \state) = \targetfunc(\state), \quad \tdummy \ge 0.
% \end{aligned}
% \end{equation}
% %
%
\begin{equation}
\label{eq:HJB_FRS}
D_{\tdummy} \vfunc(\tdummy, \state) + \ham(\tdummy, \state, \nabla \vfunc(\tdummy, \state)) = 0,~~ \vfunc(0, \state) = \targetfunc(\state),
\end{equation}
%
where $\tdummy \ge 0$. 
Here, $D_{\tdummy} \vfunc(\tdummy, \state)$ and $\nabla \vfunc(\tdummy, \state)$ denote the time and space derivatives of the value function respectively.
The function $\targetfunc(\state)$ is the implicit surface function representing the initial set of states $\targetset = \{\state: \targetfunc(\state) \le 0\}$.
The Hamiltonian, $\ham(\tdummy, \state, \nabla \vfunc(\tdummy, \state))$, encodes the role of system dynamics and control, and is given by
\begin{equation}
\label{eq:HJB_ham}
\ham(\tdummy, \state, \nabla \vfunc(\tdummy, \state)) = \max_{\hctrl \in \cset} \nabla \vfunc(\tdummy, \state) \cdot \jointdyn(\state, \hctrl).
\end{equation}

Once the value function $\vfunc(\tdummy, \state)$ is computed, the FRS is given by $\frs(\tdummy) = \{\state: \vfunc(\tdummy, \state) \le 0\}$.
% %
% \begin{equation*}
% \frs(\tdummy) = \{\state: \vfunc(\tdummy, \state) \le 0\}.
% \label{eq:frs_set}
% \end{equation*}
% % 
% HJ reachability also provides the optimal human action that maximally expands the FRS and is given by 
% %
% \begin{equation}
% \label{eq:opt_ctrl}
% \hctrl^{*}(\tdummy,\state) =  \arg \max_{\ctrl \in \cset} \min_{\dstb \in \dset} \nabla \vfunc(\tdummy, \state) \cdot \dyn(\state, \ctrl, \dstb).
% \end{equation}

%\subsection{HJ Reachability-based FRS Computation}
\subsection{An HJ Reachability-based framework for prediction \\ and analysis}
\label{subsec:hj_framework}
% \adedit{In this section, we build on the reachability formalism for prediction to obtain a framework which we will use to both generate faster predictions, as well as to enable planners to answer important analysis questions about Bayesian predictors. Our framework is based on one key idea: rather than working with a probability distribution over human actions as in (eq 11), we will use a deterministic set of allowable human actions at every step. Very importantly, the set will state-dependent, and therefore \emph{belief}-dependent:
% \begin{equation}
% \hctrl \in \cset(z),\quad \cset(z) = \{\hctrl: h(\hctrl,z)\geq \delta \}
% \end{equation}
% with $h$ some function allowed to depend on both the control and the state $z=(x_H,\beta)$ and $\delta$ some threshold. Different choices of $h$ led to different sets $\frs(\tdummy)$. The FRS can now be computed using the HJB-PDE at a significant lower computational complexity.} 

% \adedit{\noindent\textbf{Prediction.} We generate a predictor from our framework by instantiating the set of allowable human actions to be only actions that have sufficient probability under the belief: \begin{equation} \label{eqn:jointdyn_HJ_controlpolicy}
%     \hctrl \in \cset(z),\quad \cset(z) = \{\hctrl: P(\hctrl \mid \jointstate) \ge \delta\},
% \end{equation}
% The effect is that now, rather than associating future states with probabilities, what we have access to at every time step is a set of feasible states $z$. At every step, the set still evolves via eq 10, but now all actions that have too low probability are excluded, and actions that have high probability are all treated as equally likely. However, because of coupling between future belief and allowable actions, we may approximate $\frspos^{\tvar}_{\epsilon}(\tdummy)$ via a $\approxfrspos^{\tvar}_{\delta}(\tdummy)$,  obtained by using a non-zero $\delta \propto \epsilon^{\frac{1}{\gamma\tdummy}}$. The next section shows how this predictor relates to $\frspos^{\tvar}_{\epsilon}(\tdummy)$ empirically and discusses is pros and cons.} 

% \adedit{\noindent\textbf{Analysis.} Suppose we have a prior (or current belief), but we worry that the prior might be wrong, i.e. $\arg\max P(\beta)\neq \beta^*$, with $\beta^*$ being some hypothesized ground truth value for the human internal state. A reasonable question would be how long it would take the robot to realize that the value of the internal state is $\beta^*$, i.e. place enough probability in its posterior on $\beta^*$. To answer this type of questions, a different instantiation of our framework is required: we now want to compute the FRS under allowed human actions that are modeling the ground truth, and compute how long it takes to attain the desired property on the belief. Thus, the allowed control set is:
% \begin{equation} \label{eqn:jointdyn_HJ_controlpolicy_gt}
%     \hctrl \in \cset(z),\quad \cset(z) = \{\hctrl: P(\hctrl \mid x_H, \beta^*) \ge \delta\},
% \end{equation}}

% \adedit{Overall, by choosing $h$ appropriately, we can generate a range of predictors and analyses. The two examples above seemed particularly useful to us, and we detail them in the following sections. Other researchers might have a need for different instances, like allowing actions that are probable under a different distribution from $z$ or from a specific hypothesis. }\adnote{need a better way to say this, but would be good to give an example of something else the framework allows for that we wont cover}

% \adnote{the edit above would replace:}

In this section, we build on the reachability formalism for prediction in Sec. \ref{sec:stochastic_fromulation} to obtain a framework which we will use to both generate robust and faster predictions, as well as to enable planners to answer important analysis questions about Bayesian predictors. 
Our framework is based on one key idea: rather than using a probability distribution over human actions as in \eqref{eqn:jointdyn_controlpolicy}, we will use a deterministic set of allowable human actions at every step. 
Very importantly, this set will be state-dependent, and therefore \emph{belief}-dependent:
\begin{equation} \label{eqn:allowable_control_general}
\hctrl \in \cset(z),\quad \cset(z) = \{\hctrl: h(\hctrl,z)\geq \delta \}
\end{equation}
where $h$ is a function allowed to depend on both the control and the state $\jointstate=(\hstate,\param)$, and threshold $\delta$.
% The control set depends on the threshold $\delta$, which is a design parameter.
Using a control set rather than a distribution allows us to convert the stochastic reachability problem in Sec. \ref{sec:stochastic_fromulation} to a deterministic reachability problem, which can be solved using the HJB-PDE formulation in Section \ref{subsec:hj_reachability}.
% 
% Different choices of $h$ in \eqref{eqn:allowable_control_general} will lead to different sets $\frs(\tdummy)$.
We now illustrate how different instantiations of $h$ in our framework enable both robust prediction and predictor analysis.
%

\noindent\textbf{Prediction.} We generate a predictor using our framework by instantiating the set of allowable human actions to be only those with sufficient probability under the belief: \begin{equation} \label{eqn:jointdyn_HJ_controlpolicy}
    \hctrl \in \cset(z),\quad \cset(z) = \{\hctrl: P(\hctrl \mid \jointstate) \ge \delta\}.
\end{equation}
Now, instead of associating future states with probabilities, we maintain a set of feasible states $z$ at every time step. Over time, this set still evolves via \eqref{eq:joint_dynamics}, but now all actions that have too low probability are excluded, and actions that have high probability are all treated as equally likely. However, because of the coupling between future belief and allowable actions, we may approximate $\frspos^{\tvar}_{\epsilon}(\tdummy)$ via a $\approxfrspos^{\tvar}_{\delta}(\tdummy)$, using a non-zero $\delta$.
% \propto \epsilon^{\frac{1}{\gamma\tdummy}}$. 
This has two advantages: (a) when the prior is correct, this allow us to compute an approximation of $\frspos^{\tvar}_{\epsilon}(\tdummy)$ using the computational tools developed for reachability analysis, and (b) when prior is incorrect, this allows the predictions to be robust to such inaccuracies, since computation of $\approxfrspos^{\tvar}_{\delta}(\tdummy)$ no longer relies on the exact action (or observation) probabilities.
We further discuss these aspects in Sec. \ref{sec:new_predictor}.
% In Sec. \ref{sec:new_predictor}, we demonstrate how $\approxfrspos^{\tvar}_{\delta}(\tdummy)$ relates to $\frspos^{\tvar}_{\epsilon}(\tdummy)$ empirically and discuss the relative pros and cons.

\noindent\textbf{Analysis.} Suppose we have a prior (or current belief) over $\param$; however, the prior might be wrong, i.e. $\arg\max_{\param^{'}} P(\param^{'})\neq \param^*$, with $\param^*$ being some hypothesized ground truth value for the human internal state. 
A reasonable question to ask in such a scenario would be ``how long it would take the robot to realize that the value of the internal state is $\param^*$, i.e. to place enough probability in its posterior on $\param^*$?'' 
A different instantiation of our framework can be used to answer such questions: we now want to compute the \frsname{} under allowed human actions that are modeling the hypothesized ground truth, and compute how long it takes to attain the desired property on the belief (we discuss this further in Sec. \ref{sec:predictor_analysis}). 
Thus, the allowed control set is:
%
\begin{equation} \label{eqn:jointdyn_HJ_controlpolicy_gt}
    \hctrl \in \cset(\jointstate),\quad \cset(\jointstate) = \{\hctrl: P(\hctrl \mid \hstate, \param^*) \ge \delta\}.
\end{equation}
%

Overall, by choosing $h$ appropriately, we can generate a range of predictors and analyses. 
The two examples above seemed particularly useful to us, and we detail them in the following sections. 
% However, there are other possible instantiations of our framework that could be useful depending on the application.
% at hand, such as allowing human actions that are probable under a different distribution from $\jointstate$ or from a specific hypothesis.
% 
% \adnote{need a better way to say this, but would be good to give an example of something else the framework allows for that we wont cover}
% \adnote{the edit above would replace:}
% 
% 
% Since the computation of $\frs(\tdummy)$ is a stochastic reachability problem, it is computationally expensive to compute this set. 
% We approximate this set by only considering the actions that are likely above a particular threshold at state $\jointstate$, and then propagating the FRS without taking into account the probabilities of these actions, as if it were a deterministic set of control actions.
% In particular, we use the following set of controls at state $\jointstate$:
% %
% \begin{equation} \label{eqn:jointdyn_HJ_controlpolicy}
%     \hctrl \in \cset,\quad \cset = \{\hctrl: P(\hctrl \mid \jointstate) \ge \delta\},
% \end{equation}
% %
% where $\delta$ is a design parameter used for finding the support of human actions at a state, and allows us to tune the conservativeness of the resultant FRS. 
% With the control policy in \eqref{eqn:jointdyn_HJ_controlpolicy}, the FRS can now be computed using the HJB-PDE at a significant lower computational complexity; however, the trade-off is that we no longer obtain the probabilities of each human state in the FRS so we may not explicitly compute $\frspos^{\tvar}_{\epsilon}(\horizon)$ for $\epsilon > 0$. 
% However, a reasonable approximation of $\frspos^{\tvar}_{\epsilon}(\horizon)$ (denoted as  $\approxfrspos^{\tvar}_{\delta}(\horizon)$ here on) can still be obtained by using a non-zero $\delta \propto \epsilon^{\frac{1}{\gamma\horizon}}$.
% 
% \adnote{I'd move the running example to the section where we show the predictor tradeofss: what it does well, what it does differently and arguably well}


==> (ICRA 2020) Reachability for Human Motion Predictors/sections/problem_formulation.tex <==
\section{Problem Statement}
% \abnote{NOTE: should agree on if we are using belief notation $b_t$ or pdf notation $P_t$}
% \begin{itemize}
%     \item Assume known robot goal $\rgoal$, map of static parts of environment environment $\map$
%     \item Want to move $\rstate$ to $\rgoal$ without colliding with human or the static obstacles
%     \item Since we already know the environment map, but we don't know the human occupancies in the future
%     \item We will divide this problem into two steps: prediction and planning
% \end{itemize}
% 
We study the problem of safe motion planning for a mobile robot in the presence of a single human agent.
In particular, our goal is to compute a control sequence for the robot which moves it from a given start state to a goal state without colliding with the human or the static obstacles in the environment. 
We assume that both the robot and human states can be accurately sensed at all times.
Finally, we also assume that a map of the static parts of the environment is known; however, the future states of the humans are not known and need to be predicted online. 
Consequently, we divide the safe planning problem into two subproblems: human motion prediction and robot trajectory planning. 
% \adnote{it's not path if it's timed, and it needs to be timed if you are avoiding a time-moving obstacle} \adnote{I know you're worried about making it roboticsy enough for icra, but i'd say it's obvious enough that you need motion prediction to plan what the robot does (and you can point to many papers for this) that you don't really need to dedicate space in the paper to the robot planning part; it's enough to show an example at the end, where you can write a few sentences about how you did planning with this; i don't feel strongly about this, just a suggestion if space is tight}

\subsection{Human Motion Prediction with Online Updates} \label{sec:human_prediction_setup}
To predict future human states, %we employ a dynamics model of the human's physical states and a model of the human's control policy.
we model the human as a dynamical system with state $\hstate \in \R^\hxdim$, control $\hctrl \in \R^\hudim$, and dynamics
\begin{equation} \label{eqn:human_dynamics}
    \hderiv = \hdyn(\hstate, \hctrl).
\end{equation}
Here, $\hstate$ could represent the position and velocity of the human, and $\hdyn$ describes the change in their evolution over time. 
To find the likely future states of the human, we couple this dynamics model with a model of how the human chooses their actions. In general, this is a particularly difficult modeling challenge and many models exist in the literature (see \cite{rudenko2019human}). 
%For example, the control policy could be hand-engineered based on prior knowledge of how people behave \cite{XYZ}, or learned from data \cite{XYZ}. 
In this work, we primarily consider stochastic control policies that are parameterized by $\param^{\tvar}$:
% wherein at each timestep $\tvar$ the human's control action is sampled from the given control policy which is parameterized by $\param^{\tvar}$:
%
\begin{equation}
    \hctrl^\tvar \sim P(\hctrl^\tvar \mid \hstate^\tvar; \param^{\tvar}).
    \label{eq:control_policy}
\end{equation}
%
In this model, $\param^\tvar$ can represent many different aspects of human decision-making\footnote{This formulation is easily amenable to deterministic policies where $P(\hctrl^\tvar \mid \hstate^\tvar; \param^{\tvar})$ is the Dirac delta function.}, from how passive or aggressive a person is \cite{sadigh2016information} to the kind of visual cues they pay attention to in a scene \cite{kitani2012activity}. The specific choice of parameterization is often highly problem specific and can be hand-designed or learned from prior data \cite{ziebart2009planning, finn2016guided}. Nevertheless, the true value of $\param^{\tvar}$ is most often not known beforehand and instead needs to be estimated after receiving measurements of the true human behavior. Thus, at any time $\tvar$, we maintain a distribution $\ptparam$ over $\param^{\tvar}$, which allows us to reason about the uncertainty in human behavior online based on the measurements of $\hctrl$. 

\example{We now introduce a running example for illustration purposes throughout the paper.
In this example, we consider a ground vehicle that needs to go to a goal position in a room where a person is walking.
We consider a planar model with state $\hstate = [h_x, h_y]$, control $\hctrl = \theta$, and dynamics $\dot{x}_H = [v_H cos(\theta), v_H sin(\theta)]$.
%
% \begin{equation}
%     \label{eqn:example_human_dynamics}
%     \begin{bmatrix}
%     \dot{h}_x \\
%     \dot{h}_y
%     \end{bmatrix} = \begin{bmatrix}
%                 v_H cos(\theta) \\
%                 v_H sin(\theta) 
%               \end{bmatrix},
% \end{equation}
% \begin{equation}
%     \label{eqn:example_human_dynamics}
%     \dot{x}_H = [v_H cos(\theta), v_H sin(\theta)].
% \end{equation}
%
The model parameter $\param^{\tvar}$ can take two values and indicates which goal location the human is trying to navigate to. 
The human policy for any state and goal is given by a Gaussian with mean pointing in the goal direction and a variance representing uncertainty in the human action:  
    \begin{equation}
       \hctrl^{\tvar} \mid \hstate^{\tvar} \sim 
    \begin{cases}
        \mathcal{N}(\mu_1, \sigma_1^2),  & \text{if } \param^{\tvar} = g_1 \\
        \mathcal{N}(\mu_2, \sigma_2^2),  & \text{if } \param^{\tvar} = g_2
    \end{cases},
    \end{equation}
where $\mu_i = \tan^{-1}\big(\frac{g_i(y) - h_y^{\tvar}}{g_i(x) - h_x^{\tvar}}\big)$ and $\sigma_i = \pi/4$ for $i \in \{1, 2\}$. 
% Here, $\param^{\tvar}$ can take two values and indicates which goal location the human is trying to navigate to.
$(g_i(x), g_i(y))$ represents the position of goal $g_i$.
} 

Since we are uncertain about the true value of $\param^{\tvar}$, we update $\ptparam$ online based on the measurements of $\hctrl^{\tvar}$.
This observed control may be used as evidence to update the robot's prior belief $\ptparam$ about $\param^{\tvar}$ over time via a Bayesian update to obtain the posterior belief:
%
\begin{equation}
\label{eqn:bayesian_update}
\postpt(\param^{\tvar} \mid \hctrl^\tvar, \hstate^\tvar) = \frac{P(\hctrl^\tvar \mid \hstate^\tvar; \param^{\tvar})\ptparam}{\sum_{\bar{\param}}P(\hctrl^\tvar \mid \hstate^\tvar; \bar{\param})\pt(\bar{\param})}
\end{equation}
%
Given the human state $\hstate^{\tvar}$, the dynamics $\hdyn$ in \eqref{eqn:human_dynamics}, the control policy in \eqref{eq:control_policy}, and the distribution $\ptparam$, our goal is to find the likely human states at some future time, $\tvar+\tdummy$:
%
\begin{equation}
    \frspos^{\tvar}_{\epsilon}(\tdummy) = \{\hstate^{\tvar+\tdummy} \mid P(\hstate^{\tvar+\tdummy} \mid \hstate^{\tvar}) > \epsilon\},
\end{equation}
%
where $\epsilon \ge 0$ is the desired safety threshold and is a design parameter.
When $\epsilon = 0$, we drop the subscript $\epsilon$ in $\frspos^\tvar$.
Using this set of likely human states, our robot will generate a trajectory that at each future time step $\tvar+\tdummy$ avoids $\frspos_{\epsilon}^{\tvar}(\tdummy)$. 
% \adnote{because that is the use of these sets, it's not just T that matters, its 0 through T -- not sure if you want to change notation to call $K(\tau)$ or something, as T makes it seem like the full horizon.} 

% \adnote{Here would me my rephrasing of the below paragraph:}
% \adnote{[add this first sentence per intro point about our insight, as we will come back to it later when we go from stochastic to deterministic]:}
% \adedit{Note that the requirement to compute $\frspos^{\tvar}(T)$ is different from computing the full $P(\hstate^{\tvar+\horizon} \mid \hstate^{\tvar})$ distribution. For computing the full distribution, we have two options: either sum over all possible future values of $\param$: $$\sum_{\beta_{t:T}}\sum_{u_{t:T}}\prod_{\tau} P(\beta_{\tau+1}|\beta_{\tau})
% P(u_{\tau}|x_{\tau},b_{\tau})P(x_{\tau+1}|x_{\tau},u_{\tau}) $$ 
% or sum over only future human actions, but use the belief space:
% $$ \sum_{u_{t:T}}\prod_{\tau}P(b_{\tau+1}|b_{\tau})
% P(u_{\tau}|x_{\tau},\beta_{\tau})P(x_{\tau+1}|x_{\tau},u_{\tau})$$
% The latter computation can be thought of as branching on future observations, and keeping track of what the belief might be at each future time depending on that observation history: the first term in the product corresponds to an update based on the dynamics of the human internal state, whereas the second term corresponds to the observation update. Our insight is that this latter computation can be formulated as a stochastic reachability problem, but that it can simplify to a deterministic reachability problem with lower computational complexity when it only needs to (approximately) compute the set $\frspos_{\epsilon}^{\tvar}(T)$.} 

Note that the requirement to compute $\frspos^{\tvar}_{\epsilon}(\tdummy)$ is subtly different from computing the full state distribution, $P(\hstate^{\tvar+\tdummy} \mid \hstate^{\tvar})$.
For computing the full distribution, one can explicitly integrate over all possible future values of $\param$, state, and action trajectories. 
Alternatively, one can use the belief space to keep track of $\ptparam$ over time, and compute the human state distribution using the belief. 
The latter computation can be thought of as branching on future observations, and keeping track of what the belief might be at each future time depending on that observation history and the intrinsic changes in the human behavior.
Our insight is that this latter computation can be formulated as a stochastic Hamilton-Jacobi reachability problem in the joint state space of the human and belief, but that it can be simplified to a deterministic reachability problem.
This not only leads to a more robust prediction of likely future human states when the prior $\ptparam$ is not correct, but also allows us to compute an approximation of $\frspos_{\epsilon}^{\tvar}(\tau)$ with lower computational complexity when the prior is correct.
% with lower computational complexity when we only need to (approximately) compute the set $\frspos_{\epsilon}^{\tvar}(\tau)$.
% 
% 
% The computation of $\frspos^{\tvar}(T)$ is challenging for several reasons.
% First, the belief $\ptparam$ might change upon receiving new observations.\adnote{it's not clear that you need to account for that in order to make predictions for t+T; static case, do it for each beta, dynamics case, it's clear you need to compute how the initial state might change, but not that you need to account for future observations}
% Second, the human behavior itself might change intrinsically over time (for example, the human might decide to change its goal over time).
% Since $\ptparam$ affects the likely controls of the human\adnote{very importantly, the belief does *not* affect the future controls -- look at your equation 2, it's the actual value that affects it; assuming you change beta to be time-dependent too, i think you're trying to say is that to predict you either have to branch on all possible values beta can change to at every step, or keep track of what your future belief over beta will be; i have a thought for the math to write to clarify this: I think you can write how to do the prediction -- either you sum over all possible betas $$\sum_{\beta_{t:T}}\sum_{u_{t:T}}\prod_{\tau} P(\beta_{\tau+1}|\beta_{\tau})
% P(u_{\tau}|x_{\tau},b_{\tau})P(x_{\tau+1}|x_{\tau},u_{\tau}) $$ 
% or you sum only over us and do it in belief space:
% $$ \sum_{u_{t:T}}\prod_{\tau}P(b_{\tau+1}|b_{\tau})
% P(u_{\tau}|x_{\tau},\beta_{\tau})P(x_{\tau+1}|x_{\tau},u_{\tau})$$ -- i believe the two are equivalent; basically you don't need to predict future belief but it's sometimes easier than branching on all possible new betas.. if this is right, it's why you're doing belief prediction} which in turn affects the likely future states of the human, one needs to capture all possible changes in $\ptparam$ over time as well as the corresponding evolution of the likely states of the human.
% In this work, we use HJ reachability to compute $\frspos^{\tvar}(T)$. \adnote{this is underplaying it: make it sound like an actual exciting realization}
%
% \begin{itemize}
%     \item To plan a safe and efficient path in the presence of a human, the robot needs to predict the human's behavior.
%     \item The combination of the human dynamics model and a model of how the human chooses their controls can allow the robot to predict future states that the human is likely to occupy.
%     \item Let the physical state of the human be $\hstate \in \R^\hxdim$ where $\hxdim$ is the dimension of the human state space and $\hctrl \in \R^\hudim$ be the control where $\hudim$ is the dimension of the human's control.
%     \item The human is modeled by their dynamics:
%             \begin{equation}
%                 \hderiv = \hdyn(\hstate, \hctrl)
%             \end{equation}
%     \item Modelling the human control policy is non-trivial and many models exist (cite some stuff?). 
%     \item In general, this control policy could be hand-engineered based on prior knowledge of how people behave, or learned from data. 
%     \item In this work we will primarily consider stochastic control policies\footnote{This formulation is easily amenable to deterministic policies where $P(\hctrl^\tvar \mid \hstate^\tvar; \param)$ is the Dirac delta function.} wherein at ever timestep $\tvar$ the human's control action is  sampled from the given control policy:
%         \begin{equation}
%             \hctrl^\tvar \sim P(\hctrl^\tvar \mid \hstate^\tvar; \param)
%             \label{eq:control_policy}
%         \end{equation}
%     \item Here, $\param$ is a simple parametrization of the human's control policy. \item \abnote{(add in more stuff about this parametrization -- what can $\param$ represent, why is it useful, etc?)} %that
%     \item However, we are uncertain about the true value of $\param$, so we maintain a distribution over it, $P(\param)$.
%     \item  This distribution will allow us to reason about the uncertainty in human behavior online based on observed data. We will update the distribution online via measurements of $\hctrl$. More on the specific update models later. 
%     \item What we want is find the likely states that the human will be at in some future time, $T$:
%         \begin{equation}
%             \mathcal{K}(T) = \{ \hstate^T \mid P(\hstate^T \mid \hstate^0) > \epsilon\}
%         \end{equation}
% \end{itemize}
\subsection{Robot Motion Planning} \label{sec:motion_planning_setup}
We model the robot as a dynamical system with state $\rstate \in \R^\rxdim$, control $\rctrl \in \R^\rudim$, and dynamics $\rderiv = \rdyn(\rstate, \rctrl)$.
%
% \begin{equation} \label{eqn:robot_dynamics}
%     \rderiv = \rdyn(\rstate, \rctrl)
% \end{equation}
%
% The robot is operating an environment whose map is known. 
% In particular, let $\map$ represents the set of all obstacles in the environment.
% The goal of this paper is to determine a set of controls $\rctrl^{0:\finaltime}$ such that $\rstate^{\tvar} \not\in \hstate^{\tvar} \cup \map, \forall \tvar \in [0,\finaltime]$ and $\rstate^{\finaltime} = \rgoal$.
% Here, $\rgoal$ represents the goal state of the robot.
The robot's goal is to determine a set of controls $\rctrl^{0:\finaltime}$ such that it does not collide with the human or the (known) static obstacles, and reaches its goal $\rgoal$ by $\finaltime$.
In this work, we solve this planning problem in a receding horizon fashion.
Since the future states of the human are not known \textit{a priori}, we instead plan the robot trajectory to avoid $\frspos^{\tvar}_{\epsilon}(\cdot)$, the likely states of the human in the time interval $[\tvar, \tvar+\horizon]$, during planning at time $\tvar$.
% Even though conservative, this approach allows us to avoid the human at all times.
% \adnote{don't say it's conservative, because you can set your own epsilon}

\example{Our ground robot is modeled as a 3D Dubins' car with state given by its position and heading $\rstate = [s_x, s_y, \phi]$, and speed and angular speed as the control $\rctrl = [v_R, \omega]$. The respective dynamics are described by $\dot{x}_R = [v_R\cos\phi, v_R\sin\phi, \omega]$.
% %
% \begin{equation}
% \begin{aligned}
% \dot{s}_x = v_R\cos\phi,\quad \dot{s}_y = v_R\sin\phi,\quad \dot{\phi} = \omega\,, \\
% \underline{v} \le v_R \le \bar{v},\quad |\omega| \le \bar{\omega}.
% \end{aligned}
% \end{equation}
% %
At any given time $\tvar$, we use a third-order spline planner to compute the robot trajectory for a horizon of $\horizon$ (for more details, see~\cite{bansal2019combining}). 
%The spline trajectory is computed via an MPC scheme that avoids the static obstacles and the likely human positions, and navigates the robot towards the goal $\rgoal$.
%For the further details of the planner, we refer the interested readers to \cite{bansal2019combining}.
}
%
% \begin{itemize}
%     \item Let the robot state be $\rstate \in \R^\rxdim$ and the robot control be $\rctrl \in \R^\rudim$
%     \item A model of the robot's dynamics can be described via the differential equation
%         \begin{equation}
%             \rderiv = \rdyn(\rstate, \rctrl)
%         \end{equation}
%     \item We want to determine a set of controls $\rctrl^{0:T}$ such that $\rstate^t \notin \mathcal{K}(t) \cup \map, \forall t \in [0,T]$ and $\rstate^T = \rgoal$.
%     \item \example{Our ground robot is modeled with 3D state given by its position and heading $\rstate = [s_x, s_y, \phi]$ with heading as the control $\rctrl = \phi$. The respective dynamics of each agent are described by:
%         \begin{equation}
%             \begin{bmatrix}
%             \dot{s}_x \\
%             \dot{s}_y \\
%             \dot{\phi} 
%           \end{bmatrix} &= \begin{bmatrix}
%                         v_R cos(\phi) \\
%                         v_R sin(\phi) \\
%                         \omega 
%                       \end{bmatrix}
%         \end{equation}
%         }
% \end{itemize}
%
%
% \subsection{Human prediction problem.}
% \begin{itemize}
%     \item For planning purposes, the robot would like to know where the human will be at some future times $k \in [0,\predhor]$. More formally, we would like to predict:
%         \begin{equation}
%             P(\hstate_{t+k} \mid x_t), \forall k \in [0,\predhor]
%         \end{equation}
%     \item The dynamics model and the control policy can be combined to obtain a formula \item (note: we need to agree on how we are writing the prediction problem)
%     \item (note: should we talk about computational complexity of solving this full prediction problem?)
% \end{itemize}

==> (ICRA 2020) Reachability for Human Motion Predictors/sections/related_work.tex <==
\section{Related Work}
% 
% \subsection{Human modeling and prediction}
% Human motion prediction is challenging due to the complexity of human behavior and the necessity of robust and efficient predictions for robot motion planning.
% One common approach for predicting human behavior is to use pattern-based methods which learn behavioral structure from data. 
% The effectiveness of this approach has been demonstrated for inference and planning around human arm motion \cite{amor2014interaction, ding2011human, koppula2013anticipating, lasota2015analyzing, hawkins2013probabilistic}, to address the prediction problem for human drivers \cite{hawkins2013probabilistic, Schmerling2017, driggs2018robust}, as well as for pedestrians \cite{Ma_2017_CVPR, alahi2016social}.
% Another approach is to model the human as a dynamical system, along with a objective-driven model for decision-making. 
% Assuming that the human seeks to maximize this objective, the future states of the human can be inferred \cite{bai2015intention, baker2007goal, ng2000algorithms, ziebart2009planning, kitani2012activity}.
% For a detailed survey on human motion prediction, we refer the interested readers to \cite{rudenko2019human}.

% Recently, there has been a growing interest in predictors that exploit the model structure but also leverage the online data to adapt prediction performance \cite{fisac2018general, lasota2017multiple}.  
% Such approaches exploit modeled structure when measurements can be well-explained and display conservatism when observed behavior cannot be explained by the predictor's models.
% In this paper, we build on this work by leveraging a Hamilton-Jacobi reachability-based framework to compute and analyze the possible future predictions.
% 
% \begin{itemize}
%     \item Human motion prediction is challenging due to the complexity of human behavior and the necessity of robust and efficient predictions for robot motion planning
%     \item Much work exists on predicting human behavior through dynamical systems models \cite{XYZ}, pattern-based methods which learn behavioral structure from data \cite{XYZ}, or utility-driven models  which use or infer reward functions through statistical techniques \cite{XYZ, ziebart2009planning}. 
%     \item Recent interest in predictors which exploit modeled structure but also leverage data collected online to adapt prediction performance have shown promising results \cite{fisac2018general, lasota2017multiple}. \item Such approaches exploit modeled structure when measurements can be well-explained and display conservatism when observed behavior cannot be explained by the predictor's models. 
%     %\item Have multiple predictors which are each optimized and then blended to best explain the current data \cite{lasota2017multiple}
%     \item Bayesian filtering?
%     \item For a complete survey of human motion prediction see \cite{rudenko2019human}
% \end{itemize}

\subsection{(Safe) robot planning around humans}
Given a predictive model of the human, various motion planning methods can be leveraged to generate dynamically feasible and safe trajectories.


\begin{itemize}
    \item Safe robot motion planning literature (see comparison in the RSS work)
    \item Comparison with the POMDP literature (need to think about this a bit more)
\end{itemize}

\subsection{Belief space MDP}
\subsection{Stochastic Reachability}

==> sections/background.tex <==
\section{Background}
%
\subsection{Hamilton-Jacobi Reachability}
\begin{itemize}
    \item (describe stuff about HJ reachability)
    \item Recall that our goal is to determine where the human will be in the future. More formally, we want to compute the set of all states that our human dynamical system can reach from the initial set of states $\mathcal{L}$ at time $T$. 
    \item This is a \textit{forward reachable set} computation and can be mathematically written as an intial-value PDE:
    \begin{align}
        \frac{\partial V}{\partial t} + \max_{\hctrl \in \mathcal{U}} \nabla_\hstate V(\hstate,t) \cdot \hdyn(\hstate,\hctrl) &= 0 \\
        V(\hstate, 0) &= l(\hstate(0)) 
    \end{align}
    where $\mathcal{L} = \{\hstate: l(\hstate(0)) \leq 0\}$ where $\hstate(0)$ is the initial human state.
\end{itemize}

\SBnote{
\begin{itemize}
    \item Computation of BRS.
\end{itemize}
}

%
\subsection{Inference of model confidence}
% \SBnote{
% \begin{itemize}
%     \item Setting -- a new measurement is received and the model parameters are updated.
%     \item Equation to update the parameters (Bayes rule).
% \end{itemize}
% }


\begin{itemize}
    \item Although $P(\hctrl_\tvar \mid \hstate_\tvar; \param)$ gives us some modeled structure on the human's behavior, choosing a fixed value of $\param$ may not capture the true behavior we observe. 
    \item Consider the scenario where $\param$ represents if a person is moving towards the door or towards a desk. If we fix the model to always assume that humans move towards doors, then when the human actually moves towards the desk, our predictor cannot assign sufficient probability to the human moving in that direction. Generally speaking, we will assume that do not know the true value of $\param$ beforehand. 
    \item Fortunately, we can estimate the likelihood of the person's $\param$ by observing their actions and performing Bayesian inference. Since we are uncertain about the true value of $\param$, we will place a distribution over $\param$ denoted $\ptparam$ where $\tvar$ indicates that this is the prior distribution over $\param$ at timestep $\tvar$. 
    \item Once we have a distribution over $\param$, we can measure the human's action, $\hat{\hctrl}$, online and treat this as evidence about what $\param$ value best explains the person's behavior. 
    \item Our model of the human's control policy $P(\hctrl_\tvar \mid \hstate_\tvar; \param)$ will let us understand how likely it is to observe $\hat{\hctrl}$ given the current state and a particular value of $\param$. This \textit{observation model} will be used to update $P_t(\beta)$ every time we receive a measurement via a Bayesian update:
    \begin{equation}
        P_{\tvar+1}(\param \mid \hctrl_\tvar, \hstate_\tvar) = \frac{P(\hctrl_\tvar \mid \hstate_\tvar; \param)P_{\tvar}(\param)}{\sum_{\bar{\param}} P(\hctrl_\tvar \mid \hstate_\tvar; \bar{\param})P_{\tvar}(\bar{\param})}
    \end{equation}
    \item The update of the distribution given the observed data can be thought of as the ``dynamics'' of the distribution over the $\beta$ parameter, where the data is the ``input'' to the dynamics. We will derive the exact form of the continuous-time dynamics later (note: how should we introduce this?)
\end{itemize}


==> sections/intro.tex <==
\section{Introduction}
\begin{figure} [t!]
    \centering
    \includegraphics[width=0.8\columnwidth]{figs/front_fig.jpg}
    \caption{The robot models the human as walking towards one of the two goals shown in red. However, the human actually walks straight in between them. The predictions from our Hamilton-Jacobi reachability framework (center, in magenta) approximates the full probability distribution (right, in teal) while being more robust to model misspecification and less conservative compared to the naive full forward reachable set (left, in grey).}
    \label{fig:front_fig}
    \vspace{-1em}
\end{figure}

Planning around humans is critical for many real-world robotic applications. To effectively reason about human motion, practitioners often leverage predictive models of human motion during robot decision making. 
These models can be objective-driven where the human seeks to maximize an objective \cite{bai2015intention, baker2007goal, ng2000algorithms, ziebart2009planning, kitani2012activity} or pattern-based where the behavioral structure is learned from data and then used for planning around human arms \cite{amor2014interaction, ding2011human, koppula2013anticipating, lasota2015analyzing, hawkins2013probabilistic}, drivers \cite{hawkins2013probabilistic, Schmerling2017, driggs2018robust}, and pedestrians \cite{Ma_2017_CVPR, alahi2016social} (see \cite{rudenko2019human} for a detailed survey).
% 
%Such predictive models encode relevant structure in human decision-making---such as goal-seeking behavior or preferences for smooth motions---as model parameters.
Such predictive models often encode the relevant structure in human decision-making as model parameters. However, since modeling the true human behavior and how people make decisions \textit{a priori} is challenging, predictors maintain a belief distribution over these model parameters \cite{fisac2018general, lasota2017multiple}. 
This enables the predictor to use observations of human behavior during runtime to update the belief over the model parameters and probabilistically predict the human motion in accordance with the observations. 

% Unfortunately, probabilistic predictions over future human states is typically a computationally demanding task, made only more demanding if the predictive model encodes how the human's behavior\adnote{make it clear that you're referring to the internal state, and give an example to motivate why (someonemight change their goal or diriving style or what not)} may change over time; predictions now have to account for not only future observations\adnote{i find the term accounting for future observations confusing, as you have not established prediction has to account for future observations -- you've only said that predictions depend on past observations via belief, and that predictions may account for human internal state dynamics; i think here instead of account for future observations you mean reason about future actions given the current belief} but also all possible ways in which the true model parameters may evolve. 
%
Unfortunately, generating probabilistic predictions over future human states is typically computationally demanding, made only more demanding if the human behavior may change over time.
%For example, a person walking through a hallway may suddenly change course upon realizing they forgot an item of theirs.  
For example, a human driver might change how aggressive their driving style is over time, which needs to be accounted for during the predictions.
Consequently, the predictor must now reason about all possible ways in which the model parameters and the corresponding predicted future human actions may evolve, given the current belief. In practice, however, computing the full probabilistic predictions may not necessarily be required for planning. Instead, identifying a set of states that the human will occupy with sufficiently high probability can enable the robot to avoid collisions quickly and effectively using a variety of motion planning techniques that use deterministic obstacles \cite{yoder2016autonomous, koenig2005fast, bekris2007greedy, janson2018safe}. 

In this work, we formalize the human prediction problem as a stochastic reachability problem \cite{prandini2006stochastic, abate2008probabilistic, bujorianu2007new, hu2000towards} in the joint state space of the human and the belief over the predictive model parameters.
Using this formulation, the full state distribution can be computed via a stochastic forward reachable set \cite{vinod2018stochastic, abate2007computational}, which is the set of all states and beliefs that are reachable under the human policy with at least a given probability threshold.  
However, instead of computing the stochastic reachable set, we present a novel Hamilton-Jacobi (HJ) reachability-based framework for computing a deterministic approximation of the set of probable states. 
We do so by restricting the human policy to a deterministic set of allowable actions. 
This not only allows us to predict likely human states with a significantly lower computational complexity, but it also gives rise to a general framework wherein different definitions of allowable human actions can be instantiated to (a) generate predictions and (b) perform predictor analysis. 

In particular, for prediction, the allowable human actions are those that have high enough probability with respect to any given state and belief. 
Since we do not explicitly maintain the state probabilities during prediction, on one hand our framework may lead to conservative predictions. 
On the other, our predictions are not too sensitive to these probabilities and are robust to misspecified belief distributions and model parameters (see Figure \ref{fig:front_fig}). 

Our framework additionally enables predictor analysis. 
For example, a robot motion planner might need to know how long it will take the predictor to correct a wrong prior given a hypothesized ground truth value of the human model parameters, or to disambiguate between competing hypotheses. 
We can readily answer such questions by instantiating the allowable human actions (which we use for computing our reachable sets) to model specific ground truth parameters' values. 
For instance, when the model parameter represents potential human goal locations, we can compute how long it would take a predictor to realize that the human is going towards a specific goal in the scene. 
If we do this for two goals in the scene and take the maximum of those times, the robot now also knows that no matter which of the two goals the human is actually pursuing, the identity of the correct goal will become clear within that amount of time.
% 
% We can readily answer such questions by restricting allowable human actions to model the hypothesized ground truth, and compute how long  it takes the predictor to correct an incorrect prior. 
% 
% \adnote{this paragraph needs some work to both explain why restricting allowable actions to model a hypothesized ground truth relates to questions you raised, as well as to incorporate the disambigutation properly (the last sentence now talks aabout correcting a n incorrect prior only}\adnote{e.g. "how long it will take for the predictor to correct a wrong prior given a hypothesized ground truth value for human internal state, or to disambiguate between competing hypotheses. We can readily answer such questions by instantiating the allowable human actions (which we use for computing our reachable sets) to model specific ground truth internal state values. For instance, we can compute how long it would take a predictor to realize that the human is going towards a specific goal. If we do this for two goals in the scene and take the maximum of those times, the robot now also knows that regardless which of the two goals the human is pursuing, the identify of the correct goal will become obvious within that amount of time."}

\ernote{We should probably defer the following discussion of comparing our approach with POMDPs and belief state MDPs, to e.g. the journal version.} Our framework can also be thought of as a marriage between techniques from the belief space planning literature, and optimal control methods. For example, POMDPs are often recast as belief space MDPs, which in turn often admit more computationally efficient solution methods~\cite{kurniawati2008sarsop, roy2005finding, pineau2003point}. Similarly to how POMDPs can be recast as equivalent belief space MDPs, we also operate in belief space. But rather than doing both the planning and prediction in the belief space, we only do human motion prediction in the belief space, separate from planning, as is often done in the literature to reduce the computational complexity (e.g.~\cite{littman1995learning}). However, we use theoretically-rich continuous-time reachability analysis \cite{mitchell2005time, abate2008probabilistic} for prediction, which allows us to leverage a variety of tools \cite{mitchell2004toolbox, chen2013flow} developed to solve such problems grounded within the optimal control literature.  
%

To summarize, our key contributions are:
\begin{itemize}
    \item a Hamilton-Jacobi reachability-based framework for prediction generation and predictor analysis;
    \item demonstration of our approach in simulation and on a hardware testbed for safe navigation around humans.
\end{itemize}

% \abnote{Anca point: say "from the perspective of reachability people -- this is what our paper gives you. From the perspective of Bayesian prediction people -- this is what our paper gives you." We should do this both in intro and conclusion.}
% 
% \vspace{1cm}
% 
% \adnote{v0 [best of all words]}
% \begin{itemize}
%     \item planning requires human behavior prediction
%     \item human behavior is driven by human internal state: intentions, preferences; predictors can account for this by holding a belief over that internal state (cites)
%     \item this makes predicting probability distributions over future human states difficult especially if the human internal state is dynamic (e.g. if the person might change their goal): the robot has to not just account for possible future actions given an internal state, but also the possible ways in which the internal state might evolve
%     \item (all you need is a set:) often times though, what we use for safe planning is not the full probability distribution: what we care about is identifying a set of states that has high enough probability -- we want to avoid collisions with all of those, and do not necessarily need to know which states within that set are more or less probable
%     \item (insight: we can approximate the set via reachability) we observe that finding such a set of probable states is a simpler problem than finding a full distribution; our insight is that we can approximate this set by formalizing prediction as a reachability problem; this is no ordinary reachability problem though: it's one where we compute which states \emph{and beliefs} are reachable 
%   given certain assumptions on allowable human actions; 
%   \item importantly, even though we do reachability in belief space, this is still much simpler than the problem of finding the full distribution -- that'd be stochastic reachability, complexity XX, whereas ours has complexity XX
%   \item this gives us a framework: we can plug in different definitions for allowable human actions and get different results; 
%   \item 1) prediction:  by restricting allowable human actions given a state and belief to only those actions that have high enough probability with respect to that state and belief, we obtain a new predictor; we show that it approximates the set we'd obtain by first computing the full probability distribution and then selecting states with high enough probability; it sometimes differs, because it does not trust the probabilities from previous steps -- we end up with something less accurate if the human model giving us probabilities is correct, but more robust to misspecification of that model; overall, a good combination of the bayesian and the worst case! 
%   \item 2) for self-introspection: a planner might need to know how long it would take for the predictor to correct a wrong prior, or to be able to disambiguate between competing hypotheses; we can compute that using our framework by restricting the allowable human actions to have high enough probability given a specific value of human internal state,
%   \item contributions: framework, new predictor, analysis
% \end{itemize}

% v1 [prediction story, emphasizing stochastic->deterministic insight]
% \begin{itemize}
%     \item planning requires human behavior prediction
%     \item human behavior is driven by human internal state: intentions, preferences; predictors can account for this by holding a belief over that internal state (cites)
%     \item this makes predicting probability distributions over future human states difficult especially if the human internal state is dynamic (e.g. if the person might change their goal): the robot has to not just account for possible future actions given an internal state, but also the possible ways in which the internal state might evolve
%     \item (all you need is a set:) often times though, what we use for safe planning is not the full probability distribution: what we care about is identifying a set of states that has high enough probability -- we want to avoid collisions with all of those, and do not necessarily need to know which states within that set are more or less probable
%     \item (insight: we can approximate the set via reachability) we observe that finding such a set of probable states is a simpler problem than finding a full distribution; our insight is that we can approximate this set by formalizing prediction as a reachability problem; reachability enables us to compute which states and beliefs are reachable given certain assumptions on allowable human actions; we compute our predicted set by restricting allowable human actions given a state and belief to only those actions that have high enough probability with respect to that state and belief
%     \item we first cast it as a stochastic reachability, and simplify the human actions from a probability distribution to a set of allowable actions
%     \item we show that it approximates the set we'd obtain by first computing the full probability distribution and then selecting states with high enough probability; it sometimes differs, because it does not trust the probabilities from previous steps -- we end up with something less accurate if the human model giving us probabilities is correct, but more robust to misspecification of that model; overall, a good combination of the bayesian and the worst case! 
%     \item bonus: we keep track of future beliefs, so we can answer questions about what those beliefs might be under different hypotheses, e.g. how long it would take to correct a wrong prior; 
% \end{itemize}

% v2 [belief story]
% \begin{itemize}
%     \item planning requires human behavior prediction
%     \item human behavior is driven by human internal state: intentions, preferences; predictors can account for this by holding a belief over that internal state (cites)
%     \item our goal in this work is to provide a framework for reasoning about what the robot's future beliefs might be under different assumptions about human behavior; this is important in two ways: 
%     \item 1) for self-introspection: a planner might need to know how long it would take for the predictor to correct a wrong prior, or to be able to disambiguate between competing hypotheses; 
%     \item 2) for prediction itself: especially if the human internal state is dynamic (e.g. if the person might change their goal), predictions about future states depend, implicitly or explicitly, on future beliefs
%     \item insight: computing what beliefs we might reach is a reachability problem: compute reachable states and beliefs given allowable human actions; this gives us a framework: we can plug in different definitions for allowable human actions and get different results; 
%     \item by restricting human actions for a future state and belief to have high enough probability given that state and belief, we get a predictor that approximates the high enough probability future human states -- it sometimes differs, and when it does we end up with something less accurate if the human model giving us probabilities is correct, but more robust to misspecification of that model
%     \item by restricting human actions to have high enough probability given a specific value of human internal state, we can compute how long it would take for the predictor to identify that value as the correct one with high enough probability
%   \end{itemize} 

% v3 [belief story, motivation first]   
% \begin{itemize}
%     \item planning requires human behavior prediction
%     \item human behavior is driven by human internal state: intentions, preferences; predictors can account for this by holding a belief over that internal state (cites)
%     \item this makes prediction difficult, especially if the human internal state is dynamic (e.g. if the person might change their goal): predictions about future states depend, implicitly or explicitly, on future beliefs
%     \item future beliefs are also important for analyzing the predictor: computing properties like how long it would take, given the current belief which might be wrong, to realize with high enough probability that the true human internal state is x
%     \item insight: computing what beliefs we might reach is a reachability problem! [further, we don't necessarily care about with what probability we will reach those beliefs, so it can simplified to a deterministic reachability problem:] compute reachable states and beliefs given allowable human actions; this gives us a framework: we can plug in different definitions for allowable human actions and get different results; 
%     \item by restricting human actions for a future state and belief to have high enough probability given that state and belief, we get a predictor that approximates the high enough probability future human states -- it sometimes differs, and when it does we end up with something less accurate if the human model giving us probabilities is correct, but more robust to misspecification of that model
%     \item by restricting human actions to have high enough probability given a specific value of human internal state, we can compute how long it would take for the predictor to identify that value as the correct one with high enough probability
% \end{itemize}


% \adnote{high level / most important comments:}

% \begin{itemize}
%     \item \adnote{is the paper solving the prediction problem, or is the paper solving the "how to be safe but not overly safe" problem -- how to make predictions that are a bit more conservative but not too conservative, and how to figure out properties of your predictor that you can count on in planning;}
%     \begin{itemize}
%         \item \adnote{right now, the paper is written about solving the prediction problem, with the latter stuff (robust prediction to misspecification and analysis) just being bonus ("additional advantages") (also the problem statement is for the prediction problem, and the framework is solving the prediction problem -- note, the framework right now is not written as a framework, because it's a single thing -- i.e. the full on bayesian predictor, the fact that you can change it only becomes clear later in the last section on these "additional advantages");}
%         \item \adnote{ but really, we're computing the exact full bayesian predictor in the "framework", which begs the question -- is that useful on its own as the main contribution, rather than the main contribution being that we have a framework for these robustness/analysis "additional advantages"?}
%         \item  \adnote{if it is useful on its own, it'd be because it's an easier compute / possible for continuous spaces (which i don't get, because it's stochastic reachability) -- if it is useful for full on prediction, we should have the main "experiments" focus on that, i.e. show that you can compute the predictions when you couldn't before, or faster than you could before; }
%         \item \adnote{i worry we don't have that; instead, what we have is the latter stuff -- we have more robust prediction, and we have answers;}
%     \end{itemize}
       
% \item  \adnote{ to me right now, the contribution is towards the "how to be safe but not overly safe" instead; if so, we should be changing the problem statement to reflect this (by adding past the prediction problem which questions about the prediction we're trying to answer), as well as the intro and some of the language around where robust prediction and analysis get introduced        }
% \end{itemize} 

% \adnote{related: in intro and problem statement, the statement that we need to figure out what our future beliefs will be is taken for granted, but it's highly unclear why it's true; for the intro, i'd love to see a version where we make tracking future beliefs a goal in itself, motivated by a) dynamics of internal state, and b) being able to answer questions about your future belief, like when you will correct your prior if it's wrong, and when you will be able to differentiate between alternative hypotheses; then, once it's clear that we want to track future beliefs, we can say that our insight is to pose this as a reachability problem; we plug in different restrictions on what the human controls can be, and get different predictors and analysis answers out}


% Planning around humans is critical for many real-world robotic applications. 
% Generating robotic motion plans which safely avoid nearby humans is challenging since any such planning scheme needs to reason not only about the current state of the human, but also its possible \textit{future} states.
% Practitioners often leverage predictive models to reason about the human behavior which are subsequently used by the robot during decision making.
% Recently, there has been a surge of interest in predictive models that can adapt online based on observations of human behavior.
% Such predictors typically maintain a belief over the internal state of the human which enable richer predictions when certain parts of the human behavior is not known \textit{a priori} and must be inferred in real time.
% Even though powerful in their approach, such predictors also face some challenges: 
% since the predictor is adaptive, it is important to reason about how the belief itself might change due to the future observations\adnote{why????}.
% Moreover, the human internal state itself might change over time, which needs to be appropriately accounted for during the prediction.
% These challenges need to be overcome not only to predict the likely future states of the human, but also to reason about the convergence of the belief to the true human behavior in the scenarios where the predictor is either too conservative or not yet accurate enough to be trusted for the robotic decision making.

% In this work, we propose a Hamilton-Jacobi reachability-based framework that can overcome these challenges.
% Our framework simultaneously reasons about all possible changes in the predictor's belief over time due to the potential future observations or the intrinsic changes in the human behavior, and their effect on the resulting human states.\adnote{flip the last two sentences -- state the need first, then say our observation/insight is that this is a reachability problem}
% In particular, we compute a Forward Reachable Set (FRS) in the joint state space of the human and the belief, which is the set of all beliefs and human states that the predictor can deem likely under some permissible future observations\adnote{emphasize and connect to the next paragraph: by instantiating the framework with different versions of what are permissible future observations, you can generate different predictors and analyses; by restricting human future actions to only eliminate actions that are too inconsistent with the human's behavior so far, you get a predictor that is less conservative than FRS but more robust than a typical Bayesian predictor; by restricting human future actions to be consistent with a specific hypothesis you can compute how long it will take to correct a wrong prior, or how long it will take to disambiguate between two different hypotheses..} starting from the current belief and human state.
% One of the main advantages of our framework stems from the availability of a variety of modern numerical tools for computing reachable sets \cite{mitchell2004toolbox, chen2013flow}. \adnote{I think this is a little vague at this point -- maybe make the computational argument at the end, after you've made the argument that the framework is useful because it gives you different predictors and analyses}

% Once computed, this FRS gives us all possible likely future states of the human which can be used for safe planning around humans.\adnote{this downplays the fact that you can get a predictor that's in between optimistic bayes and overly-conservative full frs (which assumes worst case human--see comment above for a suggestion on how to fix this by talking about the ways to instantitate the framework)}
% Moreover, since we explicitly maintain all possible future beliefs, our framework is well equipped to answer some key questions about the predictor, such as what are the minimum and maximum times that it will take for the belief to converge to the true behavior of the human? 
% What are the corresponding future observations that the predictor must receive to arrive at such a decision?
% The answers to these questions can inform safe planning around humans.
% To summarize, our key contributions are:
%     \begin{itemize}
%         \item a Hamilton-Jacobi reachability-based framework to reason about all possible changes in a predictor and the human state in light of future observations;
%         \item demonstration of how the proposed framework facilitates human motion prediction and its analysis\adnote{its seems to refer to the motion, but actually it's about the prediction.. maybe it's about motion too..}, enabling safer planning around humans;  
%         \item demonstration of our approach in simulation and on a hardware testbed for safe autonomous navigation around humans in indoor environments.
%     \end{itemize}

% \begin{itemize}
%     \item Planning around humans is critical for many real-world robots, but it is challenging to do and has large safety implications for autonomous systems
%     \item Practitioners often leverage predictive models to reason about human behavior which are subsequently used by the robot during decision making
%     %\item However, innacuracies in predictive models can lead the robot to confidently make unsafe decisions
%     \item Recent interest in predictive models which can adapt online based on observations of human behavior has enabled richer predictions when certain parts of the human behavior is not known \textit{a priori} and must be inferred in real time
%     \item For safety purposes, it is important to reason about how the predictor itself may change over time, which is a computationally challenging problem. 
%     \item In this work, we propose a Hamilton-Jacobi reachability-based framework that simultaneously reasons about all possible changes in the predictor over time and its effect on the resulting human state predictions
%     \item This gives us all possible likely states of the human which can be used for safe planning
%     \item Furthermore, the same framework allows us to ensure safety in scenarios where the predictor is not yet accurate enough to be trusted during robotic decision-making
%     \item Finally, our framework can be applied to a variety of nonlinear continuous-time dynamics models \abnote{ask Claire about how to talk about the continualization of the $P(\param)$ dynamics}
%     %However, it is unclear how to ensure safety in scenarios where the predictor is not yet accurate enough to be trusted during robotic decision-making. Ensuring safety here becomes even more challenging due to the fact that the predictor itself may change over time.
%     \item In our reachability framework, we treat the unobserved human measurements as `input' to the system and how the predictor changes based on the data as part of the `dynamics'
%     \item To summarize, our contributions are:
%     \begin{itemize}
%         \item casting this problem in a reachability framework
%         \item demonstration of how the proposed framework facilitates predictor analysis that enables safer planning 
%         \item demonstration of our framework in simulation and hardware
%     \end{itemize}
% \end{itemize}



% \abnote{QUESTION: can we utilize or explain what $u*$ means as a result of optimizing the Hamiltonian? Would be super cool -- Anca mentions connection to legibility and that the minimum control is the most legible one}

% \abnote{Link to our project website: \href{https://abajcsy.github.io/hallucinate/}{https://abajcsy.github.io/hallucinate/}}
% \SBnote{Outline
% \begin{itemize}
%     \item Why safety is important for autonomous systems?
%     \item What is missing in the current works at a high level? -- either they don't take into account how the human behavior model might change (RSS line of work), or work under the assumption of adversarial intruder (full FRS), or consider the average case (POMDPs). Recursive planning feasibility for the robot is also not formally addressed.
%     \item What are we aiming to do in this paper (a cautiously optimistic framework -- we want to take into account our data to reduce the pessimism about the human behavior while still keeping in mind that the current belief might change in future).
%     \item How do we do it? -- we cast the belief propagation problem as a reachability problem in the state space of human and the model parameters.
%     \item Summarize the key contributions -- (a) a novel framework that bridges the gap between different approaches to safety analysis for human-robot interaction, (b) an algorithm for provably safe and recursively feasible autonomous navigation in the presence of humans, and (c) demonstrate of the framework in simulation and on a hardware testbed. 
% \end{itemize}
% }

==> sections/plan_our_approach.tex <==
\section{Our Approach: Planning}
%
\subsection{Human motion prediction for planning}
\SBnote{
\begin{itemize}
    \item Projection of the FRS on the beta dimension.
    \item Computation of the BRS for the planning purposes and why that is important.
\end{itemize}
}

%
\subsection{Safe online planning under uncertain human prediction}
\SBnote{
\begin{itemize}
    \item Planning given the states to be avoided.
    \item Update in the human model.
    \item Replanning.
    \item Lemma: Recursive feasibility.
\end{itemize}
}

==> sections/related_work.tex <==
\section{Related Work}
% 
% \subsection{Human modeling and prediction}
% Human motion prediction is challenging due to the complexity of human behavior and the necessity of robust and efficient predictions for robot motion planning.
% One common approach for predicting human behavior is to use pattern-based methods which learn behavioral structure from data. 
% The effectiveness of this approach has been demonstrated for inference and planning around human arm motion \cite{amor2014interaction, ding2011human, koppula2013anticipating, lasota2015analyzing, hawkins2013probabilistic}, to address the prediction problem for human drivers \cite{hawkins2013probabilistic, Schmerling2017, driggs2018robust}, as well as for pedestrians \cite{Ma_2017_CVPR, alahi2016social}.
% Another approach is to model the human as a dynamical system, along with a objective-driven model for decision-making. 
% Assuming that the human seeks to maximize this objective, the future states of the human can be inferred \cite{bai2015intention, baker2007goal, ng2000algorithms, ziebart2009planning, kitani2012activity}.
% For a detailed survey on human motion prediction, we refer the interested readers to \cite{rudenko2019human}.

% Recently, there has been a growing interest in predictors that exploit the model structure but also leverage the online data to adapt prediction performance \cite{fisac2018general, lasota2017multiple}.  
% Such approaches exploit modeled structure when measurements can be well-explained and display conservatism when observed behavior cannot be explained by the predictor's models.
% In this paper, we build on this work by leveraging a Hamilton-Jacobi reachability-based framework to compute and analyze the possible future predictions.
% 
% \begin{itemize}
%     \item Human motion prediction is challenging due to the complexity of human behavior and the necessity of robust and efficient predictions for robot motion planning
%     \item Much work exists on predicting human behavior through dynamical systems models \cite{XYZ}, pattern-based methods which learn behavioral structure from data \cite{XYZ}, or utility-driven models  which use or infer reward functions through statistical techniques \cite{XYZ, ziebart2009planning}. 
%     \item Recent interest in predictors which exploit modeled structure but also leverage data collected online to adapt prediction performance have shown promising results \cite{fisac2018general, lasota2017multiple}. \item Such approaches exploit modeled structure when measurements can be well-explained and display conservatism when observed behavior cannot be explained by the predictor's models. 
%     %\item Have multiple predictors which are each optimized and then blended to best explain the current data \cite{lasota2017multiple}
%     \item Bayesian filtering?
%     \item For a complete survey of human motion prediction see \cite{rudenko2019human}
% \end{itemize}

\subsection{(Safe) robot planning around humans}
Given a predictive model of the human, various motion planning methods can be leveraged to generate dynamically feasible and safe trajectories.


\begin{itemize}
    \item Safe robot motion planning literature (see comparison in the RSS work)
    \item Comparison with the POMDP literature (need to think about this a bit more)
\end{itemize}

\subsection{Belief space MDP}
\subsection{Stochastic Reachability}
